Temporal Logics on Words with Multiple Data Values

The paper proposes and studies temporal logics for attributed words, that is, data words with a (finite) set of (attribute,value)-pairs at each position. It considers a basic logic which is a semantical fragment of the logic $LTL^\downarrow_1$ of Demri and Lazic with operators for navigation into the future and the past. By reduction to the emptiness problem for data automata it is shown that this basic logic is decidable. Whereas the basic logic only allows navigation to positions where a fixed data value occurs, extensions are studied that also allow navigation to positions with different data values. Besides some undecidable results it is shown that the extension by a certain UNTIL-operator with an inequality target condition remains decidable.

==> commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%
%%                   comments                            %%
%%%%%%%%%%%%%%%%%%%%%%
%\newcounter{CommentCounter}
\newcommand{\acomment}[2]{\ \\ \fbox{\parbox{\linewidth}{{\sc #1}:\\ #2}}}
%\newcommand{\mcomment}[2]{%
%  \stepcounter{CommentCounter}%
 % {\bf$^{(\arabic{CommentCounter})}$}%
 %\marginpar{$^{({\bf{\arabic{CommentCounter}}})}${\small #1: #2}}


% with comments
\newcommand{\ahmet}[1]{\acomment{Ahmet}{#1}}
\newcommand{\thomasS}[1]{\acomment{ThomasS}{#1}}
\newcommand{\thomasZ}[1]{\acomment{ThomasZ}{#1}}
% without comments
% \newcommand{\ahmet}[1]{}
% \newcommand{\thomasS}[1]{}
% \newcommand{\thomasZ}[1]{}

\newcommand{\proofof}[1]{{\scshape\noindent Proof of #1.\quad}}


%%%%%%%%%%%%%%%%%%%%%%
%%            theorem environments              %%
%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{myclaim}{Claim}
\makeatletter 
\@ifundefined{proposition}{
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newcommand{\mysqr}[2]{{\vcenter{\hrule height.#2pt 
        \hbox{\vrule width.#2pt height#1pt \kern#1pt
           \vrule width.#2pt}
        \hrule height.#2pt}}}
\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50
  \hskip1em\hbox{}\nobreak\hfil$\mysqr{8}{8}$
  \parfillskip=0pt \finalhyphendemerits=0 \par}
  \bigskip}
\newenvironment{proof}{\noindent{\bf Proof.}\enspace}{}
\renewenvironment{proofof} [1]{\noindent{\bf Proof (of #1).}\enspace}{}
}{}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%
%%    string projections/word positions        %%
%%%%%%%%%%%%%%%%%%%%%%%

%%                for attributed words            %%%%%
\newcommand{\attword}{attributed word\xspace}
\newcommand{\attwords}{attributed words\xspace}

%%                for data words            %%%%%
\newcommand{\datastring}{data string\xspace}
\newcommand{\datastrings}{data strings\xspace}

\newcommand{\labeling}[3][\calP]{\ensuremath{#2[#3].#1}}
%\newcommand{\mdata}[3]{\ensuremath{d_{#1}(#2, #3)}}
\newcommand{\mdata}[3]{\ensuremath{#1[#3].\att{#2}}}
\newcommand{\wdat}[2]{\mdata{w}{#1}{#2}}
\newcommand{\md}[1]{\mdata{w}{a}{#1}}
\newcommand{\mda}[1]{\mdata{w'}{a}{#1}}
\newcommand{\mdaa}[1]{\mdata{w''}{a}{#1}}
\newcommand{\stringpr}[1]{\ensuremath{\textit{str}(#1)}}
\newcommand {\pos}[2]{\ensuremath{pos_{#2}(#1)}}
\newcommand {\copos}[2]{\ensuremath{copos_{#2}(#1)}}
\newcommand {\class}[2]{\ensuremath{class_{#2}(#1)}}
  
%%                for data words            %%%%%
\newcommand{\data}[2]{\ensuremath{d_{#1}(#2)}}
\newcommand{\stringproj}[2]{\ensuremath{str(#1,#2)}} 
% (zuerst wort, dann die position fï¿œr die Klasse) 
\newcommand{\classpos}[2]{\ensuremath{p_{proj}(#1,#2)}}
\newcommand{\wordpos}[3]{\ensuremath{p_{word}(#1,#2,#3)}}

%%                for strings            %%%%%
\newcommand{\symbat}[2]{\ensuremath{#1(#2)}}

%%                k-marked words            %%%%%
\newcommand{\markedw}[1]{\ensuremath{{#1}_{m}}}
\newcommand{\reducedw}[1]{\ensuremath{\textit{red}(#1)}}

%%                marking functions            %%%%%
\newcommand{\markfunction}[1]{\ensuremath{\text{Mark}_{#1}}}

%% attributed words

\newcommand {\Att}      {{\cal{ATT}}\xspace}
\newcommand {\Prop}      {{\cal{PROP}}\xspace}
\newcommand {\D}      {{\cal{D}}\xspace}
\newcommand {\nil}      {\ensuremath{nil}\xspace}


%%%%%%%%%%%%%%%%%%
%%                 Logics                      %%
%%%%%%%%%%%%%%%%%%
\newcommand{\tinm}[1]{\ensuremath{\text{#1}}}

\newcommand {\LTL}{\tinm{LTL}\xspace}
\newcommand {\classpltl}{\dataltl}
\newcommand {\sclasspltl}{\sdataltl}
% \newcommand {\ctlstar}{{$\text{CTL}^{\ast}$}\xspace}
\newcommand {\dataltl}{\tinm{BD-LTL}\xspace}
\newcommand {\frltl}{\tinm{Freeze LTL}\xspace}
\newcommand {\dataltlx}{\tinm{Basic Data LTL}\xspace}
\newcommand {\sdataltl}{\tinm{Simple Data LTL}\xspace}
\newcommand {\edataltl}[1]{\tinm{Data LTL+#1}\xspace}
\newcommand {\ddataltl}{\tinm{Data LTL$^{2}$}\xspace}
\newcommand {\xdataltl}{\tinm{XD-LTL}\xspace}
\newcommand{\freezeLTL}{\ensuremath{\text{LTL}^\downarrow_1}\xspace}
\newcommand{\diamondLTL}{\ensuremath{\text{CLTL}^\diamond}\xspace}


%%%%%%%%%%%%%%%%%%%
%%                      automata                %%
%%%%%%%%%%%%%%%%%%%

%%%%            without index          %%%%%%%%
\newcommand{\aut}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\baseaut}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\classaut}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\dataaut}[2]{\ensuremath{\langle #1, #2\rangle}}
\newcommand{\baseautinf}[1]{\ensuremath{\mathcal{#1}_{inf}}}
\newcommand{\classautinf}[1]{\ensuremath{\mathcal{#1}_{inf}}}
\newcommand{\dataautinf}[3]{\ensuremath{\langle #1, #2, #3\rangle}}


%%%%%%%%            with index          %%%%%%%%
\newcommand{\autom}[2]{\ensuremath{\mathcal{#1}_{#2}}}
\newcommand{\baseautom}[2]{\ensuremath{\mathcal{#1}_{#2}}}
\newcommand{\classautom}[2]{\ensuremath{\mathcal{#1}_{#2}}}
\newcommand{\baseautominf}[2]{\ensuremath{\mathcal{#1}_{#2}^{inf}}}
\newcommand{\classautominf}[2]{\ensuremath{\mathcal{#1}_{#2}^{inf}}}


\newcommand{\autcor}[2]{\ensuremath{\mathcal{#1}_{\text{#2}}}}
\newcommand{\autval}[2]{\ensuremath{\mathcal{#1}_{\text{#2}}}}


%%%%%%%%%%%%%%%%%%
%%             logical operators        %%
%%%%%%%%%%%%%%%%%%

%LTL operators

\newcommand{\myops}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\oname}[1]{\ensuremath{\operatorname{#1}}}
%\newcommand{\att}[1]{\ensuremath{att(#1)}}
%\newcommand{\att}[1]{\ensuremath{@\mathrm{#1}}}
\newcommand{\att}[1]{\ensuremath{@#1}}

% positional formulas
\newcommand{\X}{\myops{X}}
\newcommand{\F}{\myops{F}}
\newcommand{\Past}{\myops{P}}
\newcommand{\G}{\myops{G}}
\newcommand{\Hist}{\myops{H}}
\newcommand{\U}{\myops{U}}
\newcommand{\Y}{\myops{Y}}
\newcommand{\Since}{\myops{S}}
\newcommand{\Now}{\myops{N}}
\newcommand{\Finfty}{\ensuremath\overset{\infty}{\F}}
\newcommand{\Ginfty}{\ensuremath\overset{\infty}{\G}}

% class formulas
\newcommand{\CX}{\X^=}
\newcommand{\CF}{\F^=}
\newcommand{\CP}{\Past^=}
\newcommand{\CG}{\G^=}
\newcommand{\CU}{\oname{\U^=}}
\newcommand{\CY}{\Y^=}
\newcommand{\CS}{\Since^=}

% U bar formula

\newcommand{\Ubar}[2][]{\myops{U}^{#1}_{\att{#2}}}
\newcommand{\Sbar}[2][]{\myops{S}^{#1}_{\att{#2}}}
\newcommand{\Fbar}[2][]{\myops{F}^{#1}_{\att{#2}}}
\newcommand{\Gbar}[2][]{\myops{G}^{#1}_{\att{#2}}}
%>>>>>>> 1.72

\newcommand{\Pbar}[2][]{\myops{P}^{#1}_{\att{#2}}}
\newcommand{\Hbar}[2][]{\myops{H}^{#1}_{\att{#2}}}

\newcommand{\Xbar}[2][]{\myops{X}^{#1}_{\att{#2}}}
\newcommand{\Ybar}[2][]{\myops{Y}^{#1}_{\att{#2}}}

% U att
%<<<<<<< commands.tex
\newcommand{\Uatt}[1]{\oname{\myops{{U}_{\att{#1}}}}}
\newcommand{\Uattd}[2][\delta]{\U^{#1}_{\att{#2}}}
%\newcommand{\Uattd}[2][\delta]{\oname{{U}^{#1}_{\att{#2}}}}
\newcommand{\Satt}[1]{{\Since}_{\att{#1}}}
\newcommand{\Sattd}[2][\delta]{{\Since}^{#1}_{\att{#2}}}
%\newcommand{\Sattd}[2][\delta]{\oname{\myops{{S}^{#1}_{\att{#2}}}}}


% bar class formulas
\newcommand{\CbX}{\myops{X^{\not=}}}
\newcommand{\CbF}{\myops{F^{\not=}}}
\newcommand{\CbP}{\myops{P^{\not=}}}
\newcommand{\CbG}{\myops{G^{\not=}}}
\newcommand{\CbU}{\myops{U^{\not=}}}
\newcommand{\CbY}{\myops{Y^{\not=}}}
\newcommand{\CbS}{\myops{S^{\not=}}}

\newcommand{\C}[2][]{\myops{C}^{#1}_{\att{#2}}}
\newcommand{\Cbar}[2][]{\myops{\bar{C}}^{#1}_{\att{#2}}}
\newcommand{\multiC}[2]{\myops{C}_{\att{#1}, \att{#2}}}
\newcommand{\Ca}[1]{\myops{C'}_{\att{#1}}}
\newcommand{\Cb}[1]{\myops{C''}_{\att{#1}}}

%operators for undecidability
% alternative until operators
\newcommand{\multiD}[1]{\myops{D}_{\att{#1}}}
\newcommand{\DUe}{\myops{^* U^=}}
\newcommand{\DUue}{\myops{^{\neq}U^=}}
\newcommand{\DUeu}{\myops{^{=}U^{\neq}}}

\newcommand{\Kill}{\Now}


% non-equal data value in X^kF, k = #1, att(1) = #2, att(2) = #3
\newcommand{\nF}[3]{\myops{\F^{\att{#2} \neq \att{#3}}_{\geq #1}}}
\newcommand{\nP}[3]{\myops{\Past^{\att{#2} \neq \att{#3}}_{\geq #1}}}

% tests k = #1, att(1) = #2, att(2) = #3
\newcommand{\kXT}[3]{\att{#2} = \X^{#1} \att{#3}}
\newcommand{\kYT}[3]{\att{#2} = \Y^{#1} \att{#3}}
\newcommand{\XT}[2]{\att{#1} = \X \att{#2}}
\newcommand{\YT}[2]{\att{#1} = \Y \att{#2}}

% simple non-equal data value in X^kF, k = #1, att(1) = #2, att(2) = #3
\newcommand{\snkF}[1]{\F^{\neq}_{\geq #1}}
\newcommand{\snkP}[1]{\Past^{\neq}_{\geq #1}}
\newcommand{\snF}{\datanotF}
\newcommand{\snP}{\datanotP}

\newcommand{\skXT}[1]{\ensuremath{\X^{#1}_{=}}}
\newcommand{\skYT}[1]{\ensuremath{\Y^{#1}_{=}}}
\newcommand{\sXT}{\ensuremath{\X_{=}}}
\newcommand{\sYT}{\ensuremath{\Y_{=}}}

\newcommand{\sX}{\dataX}
\newcommand{\sY}{\dataY}
\newcommand{\sF}{\dataF}
\newcommand{\sP}{\dataP}
\newcommand{\sU}{\dataU}
\newcommand{\skF}[1]{\ensuremath{\F^{=}_{\geq #1}}}
\newcommand{\skP}[1]{\ensuremath{\Past^{=}_{\geq #1}}}

%Freeze LTL

\newcommand{\store}{{\downarrow\,}}
\newcommand{\fetch}{\ensuremath{\uparrow}}



%DataLTL operators
% \newcommand{\test}[3]{\ensuremath{v_{#1}{#2} v_{#3}}}
% \newcommand{\testknext}[4]{\ensuremath{v_{#2}\underset{#1}{#3} v_{#4}}}
% \newcommand{\testfuture}[4]{\ensuremath{v_{#2}\underset{#1}{#3} v_{#4}}}
% \newcommand{\testkprev}[4]{\ensuremath{v_{#2}\underset{#1}{#3} v_{#4}}}
% \newcommand{\testpast}[4]{\ensuremath{v_{#2}\underset{#1}{#3} v_{#4}}}
% 
% \newcommand{\equal}[3]{\ensuremath{v_{#2}\underset{#1}{\sim} v_{#3}}}
% \newcommand{\nequal}[3]{\ensuremath{v_{#2}\underset{#1}{\nsim} v_{#3}}}
% \newcommand{\equalo}[1]{\ensuremath{\underset{#1}{\sim}}}
% \newcommand{\nequalo}[1]{\ensuremath{\underset{#1}{\nsim}}}
% 
% 
% \newcommand {\multiX}[3]{\ensuremath{\X^{v_{#1}#2 v_{#3}}}}
% \newcommand {\multiF}[3]{\ensuremath{\F^{v_{#1}#2 v_{#3}}}}
% \newcommand {\multiY}[3]{\ensuremath{\Y^{v_{#1}#2 v_{#3}}}}
% \newcommand {\multiP}[3]{\ensuremath{\P^{v_{#1}#2 v_{#3}}}}
% \newcommand {\multiU}[1]{\ensuremath{\U^{v_#1}}}
% \newcommand {\multiS}[1]{\ensuremath{\U^{v_#1}}}
% 
% \newcommand{\class}[2]{\ensuremath{C_{v_{#1}}(#2)}}
% \newcommand{\classX}[2]{\ensuremath{C_{v_{#1}}(X#2)}}
% \newcommand{\classU}[3]{\ensuremath{C_{v_{#1}}(#2U#3)}}
% \newcommand{\classY}[2]{\ensuremath{C_{v_{#1}}(Y#2)}}
% \newcommand{\classS}[3]{\ensuremath{C_{v_{#1}}(#2S#3)}}
% 
%simple DataLTL operators
\newcommand{\dataU}{\ensuremath{\U^{=}}}
\newcommand {\dataX}{\ensuremath{\X^{=}}}
\newcommand{\dataS}{\ensuremath{\Since^{=}}}
\newcommand {\dataY}{\ensuremath{\Y^{=}}}
\newcommand {\knexteq}[1]{\skXT{#1}}
\newcommand {\knextneq}[1]{\ensuremath{\X^{#1}_{\neq}}}
\newcommand {\datanotF}{\ensuremath{\F^{\neq}}}
\newcommand {\datanotP}{\ensuremath{\Past^{\neq}}}
\newcommand {\dataF}{\ensuremath{\F^{=}}}
\newcommand {\dataP}{\ensuremath{\Past^{=}}}


%skipped operators
\newcommand {\multiXjump}[4]{\ensuremath{\X^{v_{#2}#3v_{#4}}_{#1}}}
%\newcommand{\multiU}[6]{\ensuremath{^{#1#2 #3}U^{4#5 #6}}}
%\newcommand{\multiS}[6]{\ensuremath{^{#1#2 #3}S^{#4 #5 #6}}}


%%%%%%%%%%%%%%%%%%%%
%%             calligraphic symbols          %%
%%%%%%%%%%%%%%%%%%%%
\newcommand {\calA}      {{\cal A}\xspace}
\newcommand {\calB}      {{\cal B}\xspace}
\newcommand {\calC}      {{\cal C}\xspace}
\newcommand {\calF}      {{\cal F}\xspace}
\newcommand {\calP}      {{\cal P}\xspace}
\newcommand {\calT}      {{\cal T}\xspace}
\newcommand {\calU}      {{\cal U}\xspace}
\newcommand {\calL}      {{\cal L}\xspace}
\newcommand {\calO}      {{\cal O}\xspace}
\newcommand {\calV}      {{\cal V}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%             technical tools for automata construction                 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\atoms}[1]{\ensuremath{\text{Cons}(#1)}}
\newcommand{\notseen}{\ensuremath{\text{nheld}}}
\newcommand{\seen}{\ensuremath{\text{held}}}
\newcommand{\marked}{\ensuremath{\text{marked}}}
\newcommand{\statusf}{\ensuremath{\text{statf}}}
\newcommand{\statusp}{\ensuremath{\text{statp}}}
\newcommand{\cl}[1]{\ensuremath{\text{cl}(#1)}}
\newcommand{\atomset}[1]{\ensuremath{\text{Conset}(#1)}}

\newcommand{\onlyonef}{\ensuremath{\text{onlyonef}}}
\newcommand{\Sone}{\ensuremath{S_\text{one}}}

% Counter Automata
\newcommand{\inc}{\ensuremath{\text{inc}}}
\newcommand{\dec}{\ensuremath{\text{dec}}}
\newcommand{\ifzero}{\ensuremath{\text{ifzero}}}

\newcommand{\ignore}[1]{}
\newcommand{\subs}{\subseteq}
\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}




\newcommand{\phieq}{\ensuremath{\rho^=}\xspace}
\newcommand{\phineq}{\ensuremath{\rho^{\not=}}\xspace}
\newcommand{\notdata}[1]{\ensuremath{\overline{\att #1}}}

\newcommand{\condname}[1]{\emph{(#1) }}
\newcommand{\lex}{\ensuremath{\vdash}\xspace}
\newcommand{\rex}{\ensuremath{\dashv}\xspace}
\newcommand{\mex}{\ensuremath{\bullet}\xspace}

\newcommand{\tatt}{\ensuremath{\text{att}}}

\newcommand{\taus}{\ensuremath{\tau_{(s)}}\xspace}
\newcommand{\psis}{\ensuremath{\psi_{(s)}}\xspace}
\newcommand{\eplus}[1][j]{\ensuremath{e^+(#1)}\xspace}
\newcommand{\eminus}[1][j]{\ensuremath{e^-(#1)}\xspace}

\newcommand{\eplussj}[1][j]{\ensuremath{e^+_{(s)}(#1)}\xspace}
%\newcommand{\eminussj}[1][j]{\ensuremath{e^-(#1)}\xspace}

\newcommand{\epluss}{\ensuremath{e^+_{(s)}}\xspace}
\newcommand{\eminuss}{\ensuremath{e^-_{(s)}}\xspace}
\newcommand{\calAs}{\ensuremath{\calA_{\psi,(s)}}\xspace}

\newcommand{\valsi}{\ensuremath{(*^i_s)}\xspace}



\newcommand{\suf}[2]{\ensuremath{suf_#2(#1)}}
\newcommand{\pre}[2]{\ensuremath{pre_#2(#1)}}



==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
We conclude by stating some questions that should be investigated
further. We would be interested to understand the exact border of
undecidability. At this point, it is not exactly clear which kinds of
intermediate and target formulas can be allowed for $\Uattd{a}$. It
would also be interesting to compare our logics with other logics that
can deal with values, particularly with guarded  $\text{LTL-FO}$ of
\cite{DeutschHull+Automatic09}. Further investigations could try to
identify fragments with more reasonable complexity and try to add more
arithmetics to the data domain.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "start"
%%% ispell-local-dictionary: "english"
%%% End: 


==> decidability-ineq.tex <==
\section{Extended Navigation}\label{sec:extended}

As already discussed before, the navigational abilities of \dataltl
are limited. It seemingly cannot\footnote{We did not attempt to find a
proof for this statement as we were aiming for an extended logic,
anyway. However, we did not find a simple way to express the property.}
 even express the simple property that for every
$p$-position $i$ there is a $q$-position $j>i$ such that
$\wdat{b}{j}\not=\wdat{a}{i}$. Furthermore, in class formulas
$\rho\dataU \tau$, the formula $\rho$ can only refer to
positions of the current class. Of course, it would be desirable to
allow more general forms of ``Until navigation''.

In this section we discuss different possibilities to extend the
navigational abilities of \dataltl in an ``Until fashion'', some of
which are decidable and some undecidable. 
In particular, we exhibit an
$\U$-operator with the ability to navigate to a position with a
different attribute value and to state some properties on (all)
intermediate positions and show that \dataltl remains decidable with
this extension. The property stated in the previous paragraph can be expressed using this operator.

The extensions we study allow formulas of the type
$\rho\Uattd{a}\tau$, where $\delta\ge 0$. Intuitively, this operator ``freezes''
the current value of attribute $\att a$ and searches for a position
$j$  such that $\tau$ holds at $j$ and $\rho$ hold
everywhere in $[i+\delta,j)$. In formulas as above,  we will refer to
$\rho$ as the \emph{intermediate formula} and $\tau$ as the
\emph{target formula}. The ``shift'' parameter $\delta$ is needed as
we aim to design a semantic
extension of simple \freezeLTL. 

Syntactically, the formulas $\rho$ and $\tau$ are positive
Boolean combinations of position formulas and positive and negative
attribute tests. More formally, we define the syntax of
\emph{U-subformulas} $\chi$ by
$
\chi ::= \varphi \mid @b \mid \notdata{b} \mid \chi \lor \chi \mid
\chi \land \chi. 
$
Intuitively, negative attribute tests $\notdata{b}$
check that attribute $b$ has a value (!) that is
different from the current frozen value. 

Thus, the semantics of  formulas $\rho\Uattd{a}\tau$, where $\rho$ and $\tau$ are $U$-subformulas, is
defined by the following additional rules.
\begin{itemize}
   \item $w,i \models \rho \Uattd{a} \tau$ if there exists a $j \geq i+\delta$ such that
$w,j,\wdat{a}{i} \models \tau$ and $w,k, \wdat{a}{i} \models \rho$ for all $k \in [i+\delta,j)$
%    \item $w,i \models \rho \Sattd{a} \tau$ if there exists a $j \leq i-\delta$ such that
% $w,j,\wdat{a}{i} \models \tau$ and $w,k, \wdat{a}{i} \models \rho$ for all $k \in (j,i-\delta]$
\item $w,i,d \models \notdata{b}$ if $\wdat{b}{i}\not\in\{\nil,d\}$. 
\end{itemize}
We simply use $\Uatt{a}$ instead of $\Uattd[0]{a}$.
We remark that  $ \rho \Uattd[-\delta]{a} \tau$, for
$\delta\ge 0$ can be expressed by
$
(\rho\Uatt{a} \tau \land \bigwedge_{i=1}^\delta \rho_i)\lor 
(\bigvee_{j=1}^\delta (\tau_j \land \bigwedge_{i=j+1}^\delta \rho_i)), 
$
where, for $k\in[1,\delta]$, $\rho_k$ and $\tau_k$ are obtained from
$\rho$ and $\tau$, respectively, by replacing every position formula
$\varphi$ by $\Y^k\varphi$, every $@b$ by $@a=Y^k@b$ and  every
$\notdata{b}$ by $\neg @a=Y^k@b$. It can be observed that this formula
has the intended meaning (that is, the semantics obtained by using
$-\delta$ in the above semantics definition). $\rho\Satt{a}\tau$ is
defined analogously.

First of all, we will see that the above mentioned restriction for
class formulas $\rho\dataU \tau$ is indeed crucial. More
precisely, if we allow positive attribute tests in the target formula
of a formula $\rho \Uatt{a} \tau$ then the logic
becomes undecidable even if the intermediate formulas are restricted
to position formulas. 

\subsection{Extended equality-navigation is undecidable}

\begin{theorem} \label{theo:undU}
Let $\calL$ denote the extension of \dataltl by the formation rule $\varphi ::=
\chi\Uatt{a}\chi$, where $\chi$ denotes $\U$-subformulas such that
\begin{itemize}
\item all intermediate formulas are position formulas and
\item all target formulas are of the form $\att a \land \varphi$ with
  a position formula $\varphi$.
\end{itemize}
Then, satisfiability of $\calL$ on finite (or infinite) \attwords is undecidable. This holds even for 1-\attwords.
\end{theorem}

\begin{proof}
  As in Theorem \ref{theo:undN}, we reduce from the non-emptiness problem for
  Minsky two counter automata. 

  As before, conditions (1) and (2) from the proof of Theorem \ref{theo:undN} can be easily expressed in \dataltl. Condition (3) can be expressed by the formula
\[
\bigwedge_{i=1}^2 \G  (\inc_i \ra (\neg \ifzero_i \Uatt{a} (\att a
\land \dec_i))).
\]



A slightly modified reduction works for infinite 1-\attwords.  
\qed
\end{proof}  


\subsection{Extended inequality navigation}

As Theorem \ref{theo:undU} does not leave much room for extensions of
$\Uatt{a}$ operators with positive attribute tests in the target
formula we focus on negative attribute tests in target
formulas. However, as 
$
\rho\Uattd{a}(\tau_1 \lor \tau_2) \equiv
(\rho\Uattd{a}\tau_1)  \lor (\rho\Uatt{a}\tau_2)
$
and position formulas are closed under conjunctions it is clearly
sufficient to consider target formulas of the form $\varphi\land
\notdata{b_1}\land \cdots\land\notdata{b_k}$. Unfortunately, at this point
our techniques can only deal with the case $k=1$.

We turn our attention now to the intermediate formulas $\rho$. We recall
that in the case of positive attribute tests in target formulas even
position formulas as intermediate formulas yield undecidability. 
In the case of (single) negative attribute tests in target formulas we
can allow arbitrary intermediate position formulas. 

Furthermore, we can add positive and negative attribute tests, but
only in a limited way. 
More precisely, we define the logic \xdataltl
by adding 
$
\varphi ::=
\chi\Uattd{a}\chi' \mid \chi\Sattd{a}\chi',
$
to the formation rules of \dataltl and requiring that
\begin{enumerate}
\item $\chi$ is restricted to formulas of the form $\rho \lor (\att b \land \phieq) \lor
(\notdata{b}\land\phineq)$  where $\phieq,\phineq$ are position
formulas and  $\phineq$ logically implies\footnote{Readers who prefer
  a syntactical criterion might think of a formula \phieq of the form
  $\varphi\lor\phineq$.} $\phieq$, and
\item $\chi'$ is restricted to formulas of the form
  $\notdata{b}\land\tau$, where $\tau$ is a position formula.
\end{enumerate}
Intuitively, $\phieq$ constrains positions where $@b$ equals the
current value of $@a$ whereas $\phineq$ constrains those where it does
not. The requirement that  $\phineq$  implies $\phieq$ is needed for
the proof of Theorem \ref{theo:SatDataPLTL}. 

Clearly \xdataltl strictly extends \dataltl and is contained in
\freezeLTL. Further it strictly extends
two-variable logic on 1-\attwords.

Following the general idea of the decidability proof for \dataltl we
first show decidability of satisfiability for 1-\attwords and reduce
the general case to this one.

\subsection{Satisfiability for \xdataltl}


\begin{theorem} \label{theo:SatDataPLTL}
Satisfiability for  \xdataltl on finite 1-\attwords is decidable. 
\end{theorem}


\begin{proof}
The proof basically extends the proof of Theorem \ref{theo:sat1bltl} for the
new formulas. As usual, we only describe the case of
$\Uattd{a}$-formulas.


Note that in the case of 1-\attwords, any additional disjunct
$\rho$ in the intermediate formula can be pushed into the disjunction
by or-ing it with both \phieq and \phineq. It thus only remains to show how to construct $\calA'_\psi$ for
formulas $\psi=(@a\land\phieq)\lor(\notdata{a}\land \phineq)\Uattd{a}(\notdata{a}\land\tau)$, where
$\phieq$ and $\phineq$ are position formulas and \phineq implies
\phieq. 



Before we describe the construction of  $\calA'_\psi$, we first
analyze the relationships between positions at which such a formula
holds. Clearly, $w,i \models (@a\land\phieq)\lor(\notdata{a}\land
\phineq) \Uattd{a}
(\notdata{a}\land\tau)$ if and only if
there is a position $j\ge i+\delta$ such that
\begin{enumerate}[(I)]
\item $w,j\models \tau$, 
\item $\mdata{w}{a}{j}\not=\mdata{w}{a}{i}$, and
\item for the minimal such $j$ every position $k\in[i+\delta,j)$ fulfills
  \begin{enumerate}[(a)]
  \item $w,k\models\phineq$ or
  \item $\mdata{w}{a}{k}=\mdata{w}{a}{i}$ and $w,k\models\phieq$.
  \end{enumerate}
\end{enumerate}


 For a given position $i$ with $w,i \models\psi$ we call the 
position $j$ of criterion (III) \emph{the $\psi$-shepherd
for} $i$. We write $H(j)$ for the herd of $j$, that is the set of positions for which $j$
is a $\psi$-shepherd (see Figure \ref{fig:ineq:def}).
%We note that it never holds $j\in H(j)$.  
A
position $j$ with $H(j)\not=\emptyset$ is also called a
\emph{shepherd}.

With each $\tau$-position $j$ we associate a set of special
positions. They are used to deal with $\psi$-positions that need
(IIIb) at least once ($\rho$-special positions) and with cases where the smallest $\tau$-position
larger than some $i$ has the same data value as $i$  ($\tau$-special positions).
\begin{itemize}
\item 
If for some $i\in H(j)$ there is a $k\in[i+\delta,j)$ such that
 $w,k\not\models\phineq$ (and thus (IIIb) holds), then we say that
 $i$ is \emph{$\rho$-far} for $j$ and $k$ is a \emph{$\rho$-stair} for $j$ and both are
\emph{$\rho$-special for $j$}.
\item If for some $i\in H(j)$ there is a $k\in[i+\delta,j)$ such that
 $w,k\models\tau$ (and due to minimality of $j$ thus
 $\mdata{w}{a}{k}=\mdata{w}{a}{i}$ holds), 
then we say that
 $i$ is \emph{$\tau$-far} for $j$ and $k$ is a \emph{$\tau$-stair} for $j$ and both are
\emph{$\tau$-special for $j$}.
\end{itemize}
We write $S(j)$ for the set of ($\rho$- or $\tau$-) special positions for $j$ and
remark that $S(j)$ does not need to be a subset of $H(j)$. See Figure \ref{fig:ineq:def} for an illustration of these definitions.

\begin{figure}
\small    $$\begin{array}{|c|*{11}{|c}|}\hline
	\text{Pos} & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\\hline
	  &  &   & \psi & \psi & & \psi & \psi &  & & \\
	 \text{Props}  & & & & \tau & & & & & &\tau \\
	   & \rho^= & & \rho^= & \rho^= & \rho^{\neq} & \rho^= & \rho^{\neq} & \rho^{\neq} & \rho^{\neq} &  \\\hline
	a & 1 & 2 & 1 & 1 & 2 & 1 & 2 & 2 & 2 & 3 \\\hline
      \end{array}$$
 \caption{For $\psi=(@a\land\phieq)\lor(\notdata{a}\land \phineq)\Uattd[2]{a}(\notdata{a}\land\tau)$, the herd of the shepherd at position $10$ is $\{3,4,6,7\}$. Position $4$ is no shepherd. Position $6$ is a $\rho$-stair for positions $3,4$. Positions $3,4$ are $\rho$-far from $10$. Positions $3,4,6$ are special for position $10$, whereas there is no special position for position $4$. Further $e^-(10) = 3$ and $e^+(10) = 6$.\label{fig:ineq:def}}
\end{figure}

For technical reasons, we define the set $S(j)$ also for 
$\tau$-positions with an empty herd. To this end, for such
$\tau$-positions $j$ we put  the maximal $k\in[j-\delta,j)$ with
$\mda{k}\not=\mda{j}$ such that
\begin{itemize}
\item all positions in $(k,j)$ are \phineq-positions, and
\item $k$ is  a $\tau$-position or it is marked by \phieq but not by \phineq
\end{itemize}
into $S(j)$, if such a position exists. Then we add all positions $\ell\in(j-\delta,k)$ with
$\mda{\ell}=\mda{k}$ to $S(j)$.


For positions $j$ with non-empty $S(j)$, we denote the minimal and maximal
special positions for $j$ by $\eminus$ and $\eplus$,
respectively (see Figure \ref{fig:ineq:def}) and call $[\eminus,\eplus]$ the \emph{special
  interval} $I(j)$ of $j$. Note that $\eplus< j$ and there is no
further $\tau$-position in $(\eplus+\delta,j)$ (as such a position
would contradict the minimality of $j$ or would be special for $j$),
thus $j$ can be easily identified, given $\eplus$. If $S(j)$ is empty, then $I(j)$ is the empty interval. By construction, if $H(j)=\emptyset$, the smallest element of $S(j)$ is larger than $j-\delta$,
thus $|I(j)|<\delta$. 



\begin{myclaim}\label{claim:s}\mbox{ }
\begin{enumerate}[({\ref{claim:s}}a)]
\item\label{claimi:unicol} All positions in
$S(j)$ have the same data value.
\item\label{claimi:eplus} For each $\tau$-position $j$  with
  $S(j)\not=\emptyset$,  $\eplus$ is the largest position $k<j$ with
  $\mda{k}\not=\mda{j}$ such that 
\begin{itemize}
\item all positions in $(k,j)$ are \phineq-positions, and
\item $k$ is  a $\tau$-position or it is marked by \phieq but not by \phineq.
\end{itemize}
\item\label{claimi:eminus} For each $\tau$-position $j$ with
  $S(j)\not=\emptyset$, $\eminus$ is the smallest position $m\le \eplus$
  with $\mda{m}=\mda{\eplus}$ such that
  \begin{itemize}
  \item all $l\in[m+\delta,j)-S(j)$ are \phineq-labeled,
  \item all $l\in[m+\delta,j)$ are \phieq-labeled,
  \item there is no $\tau$-labeled position $l\in[m+\delta,j)-S(j)$.
  \end{itemize}
\item\label{claimi:icap} $|I(j)\cap I(j')|\le \delta$ for $j\not=j'$.
\end{enumerate}  
\end{myclaim}


To show Claim (\ref{claim:s}\ref{claimi:unicol}), let $k$ be the minimal
$\rho$-far position in $S(j)$, in case $H(j)\not=\emptyset$. 
 Clearly, all $\rho$-stairs have the same value as $k$ and in turn all
 other $\rho$-far positions as well. If $H(j)=\emptyset$ then all
 positions have the same value by definition of $S(j)$. A similar argument shows that all $\tau$-special positions have
the same data value. Let now $k$ be the maximum $\rho$-stair
and $l$ the maximum $\tau$-stair in $S(j)$ and let us assume
that $\mdata{w}{a}{k}\not=\mdata{w}{a}{l}$. If $k<l$, $l$ would be a
shepherd for the smallest $\rho$-far position in $S(j)$, contradicting
the minimality of $j$. If $l<k$, then 
$\mdata{w}{a}{k}\not=\mdata{w}{a}{i}$ and $w,k\not\models\phineq$ for
the smallest $\tau$-far position, again a contradiction.

Claim (\ref{claim:s}\ref{claimi:eplus}) and
(\ref{claim:s}\ref{claimi:eminus}) basically follow directly from the definitions.

Claim (\ref{claim:s}\ref{claimi:icap}) is crucial  for the construction of $\calA'_\psi$ as it,
intuitively, implies that, for each part of the data word, there are
at most $\delta+1$ data values that
require special attention by $\calA'_\psi$.
To prove it we can assume that both $j$ and $j'$ have a
non-empty herd as otherwise one of them has an interval of size at
most $\delta$ and the claim follows trivially. 

Let therefore $j<j'$ be two shepherds. Let $i=\eminus$ , $k=\eplus$,
$i'=\eminus[j']$ and $k'=\eplus[j']$. 
We prove $i'+\delta> k$ (and thus the claim) by contradiction. To this
end, let us assume $i'+\delta\le k<j<j'$. 


\begin{figure}%[b!]
\small
    $$\begin{array}{|c|*{12}{|c}|}\hline
	\text{Pos} & i & \ldots & i'& \ldots  & i'+\delta& \ldots  & k & \ldots & j & \ldots & j' \\\hline
	\text{Spec} & e^-(j)& & e^-(j') & & & & e^+(j) & & S & &S   \\\hline
	\text{Prop} & & & & & & & & & \psi & & \psi \\\hline
	a & d' & & d & & & & d' &  & d & & \\\hline
      \end{array}$$
 \caption{Sketch for the proof of Claim (\ref{claim:s}\ref{claimi:icap}). Here, $S$ marks shepherds and $d, d'$ are two different data values. \label{fig:ineq:claim:s}}
\end{figure}

As $j'$ is the $\psi$-shepherd for $i'$,
$\mdata{w}{a}{i'}=\mdata{w}{a}{j}$ (as otherwise, because of $i'+\delta\le j$, $j'$ would not be minimal). As $j$  is the $\psi$-shepherd for $i$,
$\mdata{w}{a}{i} \not =\mdata{w}{a}{j}$. Thus, $\mdata{w}{a}{k}=\mdata{w}{a}{i}
\not =\mdata{w}{a}{j}=\mdata{w}{a}{i'}$ and therefore $i'+\delta<k$. See Figure \ref{fig:ineq:claim:s} for a sketch of the information obtained so far.  
However, if $k$
is $\rho$-special then for some $l\in[k,j)\subs[i+\delta,j)$
it holds $\mdata{w}{a}{l}=\mdata{w}{a}{k}$ and $w,l\models\phieq$
but $w,l\not\models\phineq$.  As  $\mdata{w}{a}{l}=\mdata{w}{a}{k}\not=\mdata{w}{a}{i'}$, $j'$ cannot be a
$\psi$-shepherd for $i'$, a contradiction. If, on the other hand,  $k$
is $\tau$-special then there is a $\tau$-position $j''\in[k,j)$ with
$\mdata{w}{a}{j''}=\mdata{w}{a}{k}$. But then $j''$ would be a
shepherd for $i'$, contradicting the minimality of $j'$.
This concludes the proof of Claim (\ref{claim:s}\ref{claimi:icap}).\\

To deal with the additional complication added by $\delta$, we
use additional propositions. In the intended string, each $\tau$-position
carries a proposition \taus, for exactly one $s\in\{0,\ldots,\delta\}$. The
herd of a shepherd marked by \taus  is called \emph{$s$-herd} and so on.
Besides $\taus$ we use further propositions of the form \psis, \epluss and \eminuss
with the intention that for each shepherd marked by \taus,  $\eminus$ is marked by
  \eminuss and $\eplus$ by \epluss and all positions in $H(j)$ are
  marked by \psis. We assume that all these propositions are already
  present in $w'$. However, the automaton has to test that they are as intended.

For a valid string $w'$
the assignment of $s$-values to shepherds can be done as follows. We
assign numbers $s\in\{0,\ldots,\delta\}$ in a round-robin fashion to all
positions of the form $\eplus$ and assign this $s$ to the
corresponding $\tau$-position and its herd. This guarantees that for
two positions $k=\eplussj$ and $k'=\eplussj[j']$ with $j \neq j'$ we have $|k'-k|>\delta$. 
This implies that the intervals of two distinct \taus-positions are
disjoint (as can be shown just the same way as Claim (\ref{claim:s}\ref{claimi:icap})).\\




In a nutshell, the idea for the construction of $\calA'_\psi$ is as
follows. For each  $s\in\{0,\ldots,\delta\}$ we construct an
automaton  $\calAs$ that takes care of  $s$-shepherds and their herds.
These automata independently check that for each $\taus$-position $j$ the
corresponding \eminus- and \eplus-positions are correct, and guess and check all other positions in
$S(j)$. Given the intervals, $\calAs$ checks that the $\psis$- and $\taus$-markings in $w'$ are
consistent. The construction requires some more details to control
inequality of data values sufficiently. By taking a suitable product
of these $\delta+1$ automata 
and additional auxiliary automaton (that tests, e.g., that the
\epluss-positions are numbered correctly) 
we get the automaton $\calA'_\psi$. 

In the following we describe the construction of $\calAs$ in more detail. We first
define, for each \attword $w'$ that is valid with respect to $\psi$ an extension $w''$ with
further propositions. Then we formulate some conditions that are
fulfilled by such a word
$w''$ and show how they can be checked by a data
automaton. Finally, we show that from a word $w''$ that fulfills the
conditions a word that is valid with respect to $\psi$ can be extracted. 

We use the additional propositions $\lex, \mex, \rex$ to mark special
positions in $s$-intervals 
and propositions $a^\ra,
a^\la, c^\ra, c^\la$ to enforce some data inequality conditions. More
precisely, the propositions $c^\ra$ and $c^\la$ will help to make sure
that every $s$-shepherd has a different data value from his herd and the
propositions $a^\ra$ and $a^\la$ will be used to pinpoint the $\eminuss$ positions.

To help the reader to distinguish the various kinds of propositions we
use the following conventions.
\begin{itemize}
\item We say that positions are \emph{labeled} by the propositions
  $\lex, \mex, \rex$. We call a position
that is not labeled by $\lex$, $\mex$ or $\rex$ \emph{unlabeled}.
\item We say that positions are \emph{colored} by the propositions $a^\ra,
a^\la, c^\ra, c^\la$.
\item For all other propositions we say that a position is
  \emph{marked}.
\end{itemize}


In the following the \emph{class $\delta$-predecessor} of a position
$j$ is the largest position $k\le j-\delta$ with
$\mda{k}=\mda{j}$. We call the class 1-predecessor \emph{class predecessor}


If $w'$ is a valid word (where the propositions
\taus,\psis,\eminuss,\epluss are assigned as intended), we define its extension $w''$ as follows.
\begin{itemize}
\item For every $s$-shepherd $j$, $\eminus$ is labeled by $\lex$ and
  $\eplus$ is labeled by $\rex$. All special positions between
  $\eminus$ and $\eplus$ are labeled by $\mex$.
\item Let $j$ be the minimal $\taus$-position. The
  positions in $H(j)$ are colored by $c^\ra$ and $j$ by
  $c^\la$. Then the following procedure decides the $c$-coloring for the remaining
  $\taus$-positions and their herds. Let $j$ be the smallest
  $\taus$-position whose $c^\la$-value has
  not yet been decided. Position $j$ is colored by $c^\la$ and all
  positions in $H(j)$ are  colored 
  by $c^\ra$ if and only if its class $\delta$-predecessor is \emph{not}  colored by 
  $c^\ra$ or does not exist. As the herds of different $s$-shepherds
  are disjoint this
  procedure is unambiguous. 
\item The $a$-coloring is defined similarly. 
The first $\lex$-position $k$  is  colored  by $a^\la$. All positions
strictly between $k$ and its class predecessor are colored by $a^\ra$.
Afterwards, we proceed as
  follows. The minimal $\lex$-position $k$ that is not yet decided is
  colored by $a^\la$ unless its class predecessor is colored by
  $a^\ra$. All positions strictly
between $k$ and its class predecessor which are larger than the
previous $\lex$-position are colored by $a^\ra$ if and
only if $k$ was colored by $a^\la$. Clearly, this procedure is unambiguous as well.
\end{itemize}


Next, we describe the conditions that are tested by
$\calAs=(\calB,\calC)$. For notational simplicity, we take the freedom to assume that the
additional propositions are already given in the input, that is,
$\calAs$ reads an extended word $w''$ instead of $w'$. However,
it is straightforward to translate this automaton into one in which
the base automaton  guesses additional propositions (by
means of states) and sends all propositions, encoded as states to the
class automaton.  


The first two conditions refer to the $a$- and $c$-colorings.

\begin{enumerate}[(Col 1)]
\item \condname{Consistent coloring for $\tau$}  
The class $\delta$-predecessor of a  $\taus$-position $j$ is colored by
$c^\ra$ if and only if $j$ is not colored by $c^\la$.
\item \condname{Consistent coloring for $\lex$}  
The class predecessor of a  $\lex$-position $j$ is colored by
$a^\ra$ if and only if $j$ is not colored by $a^\la$.
\end{enumerate}
We say that a position $i$ is $a$-consistent with a position $k>i$ if
$i$ is $a^\ra$-colored if and only if $k$ is $a^\la$-colored. Likewise
for $c$-consistent.

The next conditions deal with the intervals $I(j)$. 

\begin{enumerate}[(Spec 1)]
\item \condname{Global $\lex\mex\rex$ pattern}
In the whole \attword, the labeled positions respect the pattern
$((\lex\mex^*\rex)+\{\lex,\rex\})^*$. Here, a position matches
$\{\lex,\rex\}$ if both $\lex$ and $\rex$ occur.
\item \condname{Local $\lex\mex\rex$ pattern}
 In each class word, the labeled positions occur in contiguous blocks
 each of which respects the pattern
$(\lex\mex^*\rex)+\{\lex,\rex\})$.
\item \condname{Correct \rex-positions} 
A position $k$ is labeled by \rex if and only if there is a
$\taus$-position $j> k$ and 
for the minimal such position $j$
\begin{itemize}
\item all $m\in(k,j)$ are \phineq-marked and
  \begin{itemize}
  \item $k$ is not \phineq-marked or
  \item $k$ is $\taus$-marked and
    \begin{itemize}
    \item $j$ is unlabeled or
    \item $j$ is labeled and there is a $\lex$-position in $(k,j)$.
    \end{itemize}
 \end{itemize}
\end{itemize}
In this case, we call $j$ the corresponding \taus-position for $k$
(and for all other labeled positions in the interval of $k$).
\item \condname{Correct \lex-positions}
A labeled position $k$ is \lex-labeled if and only if for its
corresponding \rex-position $m$ and its corresponding
\taus-position $j$ the following conditions hold.
\begin{enumerate}[(A)]
\item all labeled positions in $(k+\delta,m]$ are \phieq-marked,
\item all unlabeled positions in $(k+\delta,m)$ are \phineq-marked,
\item  all positions in $(m,j)\cap[k+\delta,j)$ are \phineq-marked, and
\item 
one of the following conditions holds.
\begin{enumerate}[({D}i)]
\item There is a position $i<k$ such that $i+\delta<j$, $i+\delta$
  is an unlabeled $\tau$-position and all positions in $(i,k)$ are $a$-consistent
  with $k$.
\item There is a position $i<k$ such that $i+\delta<j$, $i+\delta$
  is not a $\phieq$-position and all positions in $(i,k)$ are $a$-consistent
  with $k$.
\item There is a position $i<k$ such that $i+\delta<j$, $i+\delta$ is unlabeled
  and not marked \phineq and all positions in $(i,k)$ are $a$-consistent
  with $k$.
\item None of (i)-(iii) holds and all position $<k$ are $a$-consistent
  with $k$.
\end{enumerate}
\end{enumerate}
\end{enumerate}

Finally, the following two conditions shall guarantee the validity of
$w''$ with respect to $\psi$.

\begin{enumerate}[(Log 1)]
\item \condname{Unlabeled $\psis$-positions} An unlabeled position $i$
  is marked by $\psis$ if and only if there is a
  $\taus$-position $j\ge i+\delta$ and for the minimal such position
 it holds that every  $k\in[i+\delta,j)$ is marked by $\phineq$.  If
 so, $i$ is $c$-consistent with $j$. 
\item \condname{Labeled $\psis$-positions} A labeled position $i$ is
  marked by $\psis$ if and only if there is a  $\taus$-position
  $j\ge i+\delta$  after $i$'s corresponding
  $\rex$-position $l$ and, for the minimal such $j$, every  $k\in[i+\delta,l]$ is marked by $\phineq$ or is labeled
  and marked by \phieq and every
  $k\in[l,j)\cap[i+\delta,j)$ is marked by $\phineq$.
If so, $i$ is $c$-consistent with $j$.
\end{enumerate}

Conditions (Col 1), (Col 2) and
(Spec 2) express properties of the class words of $w''$ whereas the
remaining conditions express properties of its word projection. Each
of these properties can be easily expressed in first-order logic and
can therefore be checked by the class automaton or the base
automaton, respectively. To test (Col 1) it is important that from the
propositions $=_r$ it can be easily inferred how many positions are in
the class word between a position $j$ and its class
$\delta$-predecessor. Remember that $=_r$ is holds at position $i$ if and only if $\mdata{w}{a}{i} = \mdata{w}{a}{i+r}$ (see proof of Theorem \ref{theo:sat1bltl}). 

We claim that the \attword $w''$ constructed above fulfills all Col-,
Ex- and Log-conditions if $w'$ is valid with respect to $\psis$. 
For (Col 1) this is because  every
shepherd is marked by $c^\la$ exactly if its class $\delta$-predecessor is not
colored by $c^\ra$ or does not exist at all. Likewise for (Col 2) and
\lex-positions. (Spec 1) holds because the intervals $I(j)$ are
disjoint. (Spec 2) follows from the way the $\lex \mex \rex$ labelings
are obtained from the intervals. (Spec 3) holds by the definition of
$\eplus$. (Spec 4) holds because the \lex-positions are exactly the
positions \eminus and by the construction of the $a^\ra$-coloring. 


That (Log
1) and (Log 2) hold follows from the validity of $w'$ with respect to
$\psis$ and the way the
$c^\ra$-marking is chosen.


Before we prove correctness for the automaton defined along these
lines, we show the following useful claim

\begin{myclaim}\label{claim:ints}
Let $w''$ be a 1-\attword that fulfills  all Col-,
Ex- and Log-conditions and which is valid with respect to all
subformulas of $\psi$. Then for each \taus-position $j$ the following conditions hold.
  \begin{enumerate}[({\ref{claim:ints}}a)]
  \item \label{claimi:borders} There is a \rex-labeled position $k$ for
    which $j$ is the corresponding \taus-position if and only if
    $S(j)\not=\emptyset$. If so, there is also a corresponding
    \lex-position $l$, $k=\eplus$ and $l=\eminus$.
  \item \label{claimi:borers} $S(j)$ is exactly the set of labeled points between the \lex
    and \rex-position corresponding to $j$.
 \end{enumerate}
\end{myclaim}
The part of Claim (\ref{claim:ints}\ref{claimi:borders}) concerning
\eplus follows directly from (Spec 3), (Col 1) and (Log 2). This implies in particular that
all labeled positions in some interval have a different data value
than their corresponding \taus-position. 

To show that $l=\eminus$ we
have to show that (1) $l\in S(j)$ and (2) there is no smaller $l'\in
S(j)$. By (Spec 1,2) all corresponding labeled positions have the same
data value. Therefore (Spec 4 A-C) guarantee that $l\in S(j)$. For the
sake of a contradiction let us now assume that there is $l'\in S(j)$
with $l'<l$. As $\mdaa{l'}=\mdaa{l}$, $l'$ is not $a$-consistent with
$l$. By (Spec 4 D) therefore one of the following statements holds, each
leading to a contradiction.
\begin{enumerate}[(1)]
\item  There is an position $i\in[l',l)$ such that $i+\delta<j$ and $i+\delta$
  is an unlabeled $\tau$-position. But then $i+\delta$ is a
  $\psi$-shepherd for $l'$ contradicting the minimal choice of $j$.
\item There is a position $i\in[l',l)$ such that $i+\delta<j$ and $i+\delta$
  is not a $\phieq$-position. This contradicts $l'\in S(j)$.
\item There is a position $i\in[l',l)$ such that $i+\delta<j$ and $i+\delta$ is unlabeled
  and not marked \phineq.  This also contradicts $l'\in S(j)$.
\end{enumerate}

\ignore{
\thomasS{Alt:\\
{\noindent\bf Claim 2.} 
  Let $w''$ be a 1-attributed word fulfilling all  Col-, Ex- and
Log-conditions. Then the following holds.
\begin{enumerate}[(a)]
\item If a position $i$ is strictly between a $\lex$-position $k$ and its
  corresponding $\rex$-position $l$ then $i$ is labeled if and only if
  $\mdaa{i}=\mdaa{k}$ ($=\mdaa{l}$).
\item There is no unlabeled $\taus$-position  between a $\lex$-position and its
  corresponding $\rex$-position.
\item There is no $\rex$-position strictly between a $\rex$-position $i$
  and the smallest $\taus$-position $\ge i+\delta$.
\end{enumerate}
Claim (2a) follows from (Spec 1) and (Spec 2) and Claim (2b) by (Ex
4). Claim (2c) follows from (Spec 3) as the intermediate  $\rex$-position
is not marked by \phineq (or would otherwise be marked by \taus).
}
}

Before we show that the automaton $\calA'_\psi$ is indeed correct, we
make precise what it means that a 1-attributed word $w''$
is valid with respect to \psis for a formula \[
\psi= (@a\land\phieq)\lor(\notdata{a}\land
\phineq) \CbU
(\notdata{a}\land\tau).
\] 
This is the case if for every position $i$ of $w''$ it holds that $i$ is
marked by $\psis$  if and only if 
\begin{itemize}
\item[\valsi] 
there is a position $j\ge i+\delta$ such that
\begin{enumerate}[(I')]
\item $j$ is marked by $\taus$, 
\item $\mdaa{j}\not=\mdaa{i}$, and
\item for the minimal such $j$ every position $k\in[i+\delta,j)$ fulfills
  \begin{enumerate}[(a)]
  \item $k$ is marked by $\phineq$ or
  \item $\mdaa{k}=\mdaa{i}$ and $k$ is marked by $\phieq$.
  \end{enumerate}
\end{enumerate}
\end{itemize}


We show now that if a 1-attributed word fulfills the Col-, Ex- and
Log-conditions above then each of its positions $i$ is marked by
$\psis$ if and only if \valsi holds. 

We first show that all $\psis$-positions $i$ fulfill \valsi.

We first consider the case that $i$ is unlabeled. Let $j$ be the
corresponding position guaranteed by (Log 1). Clearly $i$ and $j$
fulfill (I') and (III'). We have to show that
$\mdaa{i}\not=\mdaa{j}$. To this end, let $k\in[i,j-\delta]$ be
maximal with $\mdaa{k}=\mdaa{i}$.
\begin{itemize}
\item 
If $k$ is unlabeled then $k$
fulfills the condition of (Log 1) and is thus also labeled by
\psis. Furthermore, it is $c$-consistent for $j$ and therefore
$\mdaa{j}\not=\mdaa{k}=\mdaa{i}$.
\item 
If $k$ is labeled, there must be a \lex-position $l\in(i,k]$. As
$\mdaa{i}=\mdaa{k}=\mdaa{l}$, $i$ is not $a$-consistent with
$l$. By (Spec 4D) it follows again the existence of an intermediate
position as in (1)-(3) in the proof of Claim
(\ref{claim:ints}\ref{claimi:borders}) and as there we get the desired
contradiction.
\end{itemize}

We next   consider the case that $i$ is labeled. Let $j$ be the
corresponding position guaranteed by (Log 2). Clearly $i$ and $j$
fulfill (I') and (III') (as all labeled positions in $[i+\delta,l]$
have the same data value as $i$). Again, we have to show that
$\mdaa{i}\not=\mdaa{j}$. Let $l$ be the \rex-position corresponding to
$i$, thus $l\in[i,j)$.
\begin{itemize}
\item 
If $j$ is labeled (Spec 3) guarantees that
there is a \lex-position $m\in(l,j)$. As $j$ is the first
\taus-position after $l$ there cannot be any other $s$-interval
between $l$ and $m$. (Spec 5) and (Col 2) now guarantee
$\mdaa{l}\not=\mdaa{m}$ and thus
$\mdaa{i}=\mdaa{l}\not=\mdaa{m}=\mdaa{j}$.
\item If $j$ is unlabeled then $\mdaa{j}\not=\mdaa{l}=\mdaa{i}$
  because $j$ is the corresponding \taus-position for $l$.
\end{itemize}

Finally, we show that all positions $i$ fulfilling \valsi are marked
by \psis.

Again, we consider first the case that $i$ is unlabeled.  In this case
$i\not\in S(j)$. Therefore all intermediate positions
$k\in[i+\delta,j)$ fulfill \phineq. Therefore (Log 1) implies that $i$
is marked by \psis.

If, on the other hand, $i$ is labeled, $i\in S(j)$. Let $l=\eplus$,
i.e., the corresponding \rex-position of $i$. As all labeled positions
in $[i+\delta,l]$ have the same data value as $i$, these positions
fulfill the corresponding statement in (Log 2). Let us assume there is
a position $m\in(l,j)\cap[i+\delta,j)$ that is not \phineq-marked and
fulfills $\mdaa{m}=\mdaa{i}$. But then $m$ is a $\rho$-stair for $i$ and
therefore $m\in S(j)$. Thus, (Log 2) ensures that $i$ is \psis-marked.
This completes the proof. \qed
\end{proof}


By a straightforward extension  of the proof of Theorem
  \ref{theo:ltlmanyd} we get the following.
\begin{theorem} \label{theo:SatDataPLTL}
Satisfiability for  \xdataltl on finite \attwords is decidable. 
\end{theorem}


\begin{proof}
  It suffices to show that the construction of the proof of Theorem
  \ref{theo:ltlmanyd} can be extended for formulas of the new kind. To
  this end, we extend $t$ as follows. 


\begin{multline*}
 t\bigg((\rho \lor (\att a_i \land \phieq) \lor (\notdata{a_i}\land
 \phineq) \Uatt{a_j} (\notdata{a_k} \land \tau)\bigg):= \\
t_j\bigg((t(\rho)\lor\neg \tatt_i)\lor(\att a\land R \land t(\phieq))
\lor (\notdata{a}\land R \land t(\phineq)) \Uatt{a} (\notdata{a}\land
R\land \tatt_k \land t(\tau))\bigg)\\
\end{multline*}
\qed
\end{proof}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "start"
%%% ispell-local-dictionary: "english"
%%% End: 


==> decidability.tex <==

\section{Decidability of \dataltlx} \label{sec:decidability}

In this section we show that satisfiability for \dataltl
over \attwords is decidable. 
The proof is by a reduction to the satisfiability problem for
\classpltl over   1-\attwords (Subsection \ref{sec:multDimDecidable})
and a reduction of the latter to non-emptiness of data automata
(Subsection \ref{sec:oneDimDecidable}). In Subsection \ref{sec:infdecidable} we extend our decidability result to
$\omega$-words.
%\ahmet{Die Definition von attributed $\omega$-words müsste jetzt wieder reinkommen.}
In Subsection \ref{sec:undecidability} we show undecidability for two
extensions of \dataltl.


\subsection{\dataltlx over 1-\attwords is decidable} \label{sec:oneDimDecidable}
\ignore{
In this section we restrict our attention  1-\attwords although we will often refer to them simply by \textit{\attwords}. When we say in this section \textit{a \dataltl formula $\varphi$ is satisfiable} we mean that there exists a 1-\attword satisfying $\varphi$.  

We introduce some useful notations in the style of \ref{baseDef}. Given a simple \attword or a string projection $w$ we refer to the label at position $i$ by $\labeling{w}{i}$. The data value of position $i$ on a simple \attword  $w$ is denoted by $\data{w}{i}$. 
Given a simple \attword $w$ and a data value $d$ occurring in $w$ the \textit{class} of $d$ is the maximal set of positions $i_1 < \ldots < i_m$ with 
$\data{w}{i_j} = d$ for all $1 \leq j \leq m$. The \textit{class string} $\labeling{w}{i_1} \ldots \labeling{w}{i_m}$ of $d$ in $w$ is denoted by $\stringproj{w}{d}$. Given a position $i$ on $w$ and the class $\{i_1,  \ldots , i_m\}$ of $\data{w}{i}$ the class position $i_k$ with $i_k = i$ is denoted by $\classpos{w}{i}$.
On the other hand, with $\wordpos{w}{d}{k}$ we refer to position $i_k$ on the whole simple \attword.
\ahmet{Bezüglich $\markfunction{k}$ müssen wir noch Thomas' Kommentar berücksichtigen}
Let $\markfunction{k}$ be the set of all boolean functions $m: \{ 1,\ldots , k\} \rightarrow \{ 0, 1\}$. A \textit{k-marked simple \attword} $w  = {(\sigma_1,m_1) \choose d_1}\cdots {(\sigma_{n},m_{n}) \choose d_{n}}$ over $\Sigma$ is a simple \attword such that each position carries a datum from $D$ and a tupel $(a_i,m_i)$ with $a_i \in \Sigma$ and 
$m_i \in \markfunction{k}$. The \textit{marking} of  $w$ is \textit{correct} if
$m_i(l)=\begin{cases}
0,  & \text{if } i+l > n \text{ or } d_i \neq d_{i+l}\\
1, & \text{if } i+l \leq n \text{ and } d_i = d_{i+l} 
\end{cases}$.
Given a $k$-marked simple \attword $w$ the simple \attword obtained by removing the boolean functions from the labels of $w$ is denoted by $\reducedw{w}$.   
}

The proof of decidability of  satisfiability over   1-\attwords uses
register automata (we follow \cite{BjorklundS10}) and data automata
\cite{BojanczykMSSD2006}. Non-emptiness for data automata is decidable
\cite{BojanczykMSSD2006}. They are strictly more expressive than
register automata and for every register automaton an equivalent data
automaton can be effectively constructed \cite{BjorklundS10};
furthermore data automata are closed under intersection, union and
letter-to-letter-projection \cite{BojanczykMSSD2006}.

\paragraph*{Register Automata} 

In \cite{KaminskiF94} Kaminski and Francez introduced \textit{Finite-Memory Automata} which work on sequences of data values only but their generalization to 1-\attwords is straightforward. These automata have later been studied in \cite{DemriLazicLTL09} and \cite{NevenSV04} where they are called \textit{Register automata}. Register automata are equipped with a constant number of registers in which they can store data values which can later be compared with the data value of the current position. We refer to the definition in \cite{BjorklundS10}.

A register automaton over a finite alphabet $\Sigma$ is a tuple $\mathcal{R} = (\Sigma, S, s_0, k, \tau_0, \pi, F )$, where Q is a finite set of states, $s_0$ is the initial state, $k$ is the number of registers, $\tau_0 : \{1, . . . , k\} \rightarrow \{\bot\}$ is the initial register assignment ($\bot \notin \D$ indicates an empty assignment),
$\pi$ is a finite set of transitions and $F \subseteq S$ are the accepting states. 
The transition set $\pi$ consists of \textit{compare transitions} $(i,s,\sigma) \rightarrow s'$ and \textit{store transitions} 
$(s,\sigma) \rightarrow (s',i)$, for $i \in \{1,...,k\}, s,s' \in S$, and $\sigma \in \Sigma$. 

A configuration of $\mathcal{R}$ is a pair $(s,\tau)$, where $s \in S$ and $\tau : \{1,...,k\} \rightarrow \D \cup \{\bot\}$ is a register assignment. The initial configuration is $(s_0,\tau_0)$. A \textit{read transition} $(i, s, \sigma) \rightarrow s'$ can be applied if the current state is $s$, the next input set is $\sigma$ and the next input data value is already stored in register $i$. It takes the automaton from configuration 
$(s, \tau)$ to $(s', \tau)$. A write transition $(s, \sigma) \rightarrow (s', i)$ can be applied if the current state is $s$, the next input symbol is $\sigma$ and the next input data value $d$ is currently not stored in any register. It takes the automaton from a configuration $(s,\tau)$ to $(s',\tau')$, where $\tau'(i) = d$, and 
$\tau'(j) = \tau(j)$ for all $j \neq i$. 

A run of register automaton over $\Sigma = 2^{\calP}$ with $\calP \subseteq \Prop$ on an 1-\attword $w$ with $|w|=n$ is a sequence $(s_0, \tau_0), \ldots , (s_n, \tau_n)$ of configurations, defined in the obvious way. An \attword $w$ is accepted by a register automaton $\mathcal{R}$ if there exists a run 
$(s_0, \tau_0), \ldots , (s_n, \tau_n)$ of $\mathcal{R}$ on $w$ with $s_n \in F$.  

\paragraph*{Data Automata}

\textit{Data automata} were introduced in \cite{BojanczykMSSD2006} and have later been studied in, e.g., \cite{BjorklundS10}. 

A data automaton $\aut{A} = \dataaut{\baseaut{B}}{\classaut{C}}$ over a finite alphabet $\Sigma$ consists of a \emph{base automaton}  $\baseaut{B}$ and a \emph{class automaton} $\classaut{C}$. 
\begin{itemize}
\item $\baseaut{B} = \langle \Sigma, \Gamma_{\baseaut{B}},  S_{\baseaut{B}}, {s_0}_{\baseaut{B}},\pi_{\baseaut{B}},F_{\baseaut{B}}  \rangle$ is a nondeterministic letter-to-letter string transducer with input alphabet $\Sigma$, output alphabet 
$\Gamma_{\baseaut{B}}$, an initial state ${s_0}_{\baseaut{B}} \in S_{\baseaut{B}}$, a transition relation $\pi_{\baseaut{B}} \subseteq S_{\baseaut{B}} \times \Sigma \times \Gamma_{\baseaut{B}} \times S_{\baseaut{B}}$ and a set $F_{\baseaut{B}} \subseteq S_{\baseaut{B}}$ of accepting states. In each step $\baseaut{B}$ replaces the current label $\sigma \in \Sigma$ with a symbol $\gamma \in \Gamma_{\baseaut{B}}$.
\item $\classaut{C} = \langle \Gamma_{\classaut{B}},Q_{\classaut{C}}, {s_0}_{\classaut{C}},\pi_{\classaut{C}},F_{\classaut{C}}  \rangle$ is a nondeterministic string automaton with input alphabet $\Gamma_{\classaut{B}}$, an initial state ${s_0}_{\baseaut{C}} \in Q_{\baseaut{C}}$, a transition relation $\pi_{\baseaut{C}} \subseteq S_{\baseaut{C}} \times \Gamma_{\baseaut{B}} \times S_{\baseaut{C}}$ and a set $F_{\baseaut{C}} \subseteq S_{\baseaut{C}}$ of accepting states.
\end{itemize}
An 1-\attword $w$ of length $n$ is accepted by $\aut{A} = \dataaut{\baseaut{B}}{\classaut{C}}$ over $\Sigma = 2^{\calP}$ where $\calP \subseteq \Prop$ if there is an accepting run of $\aut{B}$ on $\stringpr{w}$, yielding an output string $\gamma_1 \ldots \gamma_n$,	such that, for each set $\pos{d}{w} = \{i_1,...,i_k\} \subseteq \{1,...,n\}$ of class positions with $d$ occurring in $w$ and $i_1 < \ldots < i_k$ the class automaton accepts $\gamma_{i_1} \ldots \gamma_{i_k}$.

We denote the set of words accepted by a data or register automaton $\aut{A}$ by $\calL(\aut{A})$. 

% The decidability of the satisfiability problem for \classpltl on 1-\attwords is by reduction to data automata.
\ignore{
For every \classpltl formula $\varphi$ we can construct a data automaton $\autom{A}{\varphi} = \dataaut{\baseaut{B}}{\classaut{C}}$ which accepts exactly the simple \attwords satisfying $\varphi$. Let $k$ be the highest number such that $\knexteq{k}$ occurs in $\varphi$. By \ref{lemma:kmarked} we can assume that $\autom{A}{\varphi}$ reads correctly $k$-marked simple \attwords. The construction of $\autom{A}{\varphi}$ is an extension of the automata construction for classical LTL with past operators (\cite{LichtensteinPZ85}). Informally speaking, the base automaton $\baseaut{B}$ labels every position $i$ of the input word $w$ with all subformulas of $\varphi$ which he guesses to hold on position $i$. The validity of formulas like $\X \psi$, $\Y \psi$, $\psi_1 \U \psi_2$ or $\psi_1 \Since \psi_2$ which refer to the navigation on the string projection of $w$ is checked by $\baseaut{B}$. The class automaton $\classaut{C}$ checks the validity of formulas like $\dataX \psi$, $\dataY \psi$, $\psi_1 \dataU \psi_2$ or $\psi_1 \dataS \psi_2$ which describe the navigation on a current class. To check formulas of the form $\knexteq{l}$ with $l \leq k$ the base automaton uses the marking functions of $w$. Formulas of the form $\datanotF \psi$ or $\datanotP \psi$ are handled by $\baseaut{B}$ and $\classaut{C}$ in joint work. For every subformula $\datanotF \psi$ of $\varphi$ the base automaton $\baseaut{B}$ marks every position which is the last position in the current class on which $\psi$ holds. Using these markings he decides for every position whether $\psi$ never holds in the future, holds only once, or at least in two different classes. The class automaton $\classaut{C}$ on the other hand assures that the markings are correct and checks for every position on which $\datanotF \psi$ is supposed to hold that $\psi$ holds in at least two different classes in the future, and if only in one class then not in any (strict) future position of the current class. Formulas of the form $\datanotP \psi$ are treated analogously except that for every class the first position on which $\psi$ holds is marked.                   
}
\begin{theorem} \label{theo:sat1bltl}
Satisfiability for  \dataltl on 1-\attwords is decidable. 
\end{theorem}
\begin{proof}
Let $\varphi$ be a \classpltl formula over a proposition set $\calP$ and the 
attribute set $\{ a \}$. 

In the following we often call 1-\attwords simply \emph{words}. 
Our automata will expect instead of words $w$ over \calP extended words
$w'$ with additional propositions. First, $w'$ allows the subformulas of $\varphi$ as
 propositions.  The intention is that a position $i$ of $w'$ is marked with
 $\psi$ if and only if $w,i\models \psi$. Furthermore,  we use propositions $=_r$ for every $r \in \{-N, \ldots, -1, 1, \ldots,
N\}$, for some $N$ that is at least as large as every $\delta$
occurring in $\varphi$. Proposition $=_r$ shall hold at position $i$ if and
only if $\md{i}=\md{i+r}$. Whether these propositions are correct in a
given $w'$ can be easily tested by a register automaton.


We call an extended  word $w'$ 
\emph{valid} if the propositions $=_r$  are as intended and each 
position $i$ carries exactly those formulas 
holding at $i$ in $w$. 
The word $w'$ is \emph{valid with respect to a
subformula} $\psi$ of $\varphi$ if $\psi$ is a proposition or $w'$ is consistent with respect to
the maximal strict subformulas of $\psi$. As an example, a word is valid with respect
to $\varphi = \varphi_1 \U \varphi_2$ if for each $\varphi$-position
$i$ there is a $\varphi_2$-position $j\ge i$ such that all positions
$k$, $i\le k<j$ are marked by $\varphi_1$. 

Clearly, each word $w$ has a unique valid extension. 
Thus, $\varphi$ is satisfiable if and only if it has a valid
extension $w'$ in which position 1 carries the proposition $\varphi$.

We show in the following that from a \classpltl formula a data
automaton $\calA_\varphi$ can be constructed that checks whether an
extended word $w'$ is valid. The statement of the theorem then follows from the
decidability of non-emptiness of data automata.

To this end, we construct for each subformula $\psi$
of $\varphi$ a data (or register) automaton $\calA'_\psi$ that decides
whether a given word is valid with respect to $\psi$ \emph{under
the assumption that it is valid with respect to all strict subformulas of
$\psi$}. By intersecting all these automata and intersecting the
result with a register automaton that tests that the $=_r$
propositions are correct and an automaton that tests whether position
1 carries $\varphi$, we obtain $\calA_\varphi$.

% We never evaluate
% formulas in extended words. Thus there should be no confusion
% between formulas (evaluated on $w$) and propositions (with the same
% name) in $w'$. 
The construction of $\calA'_\psi$ is straightforward for formulas of
the types
$
 p \mid \neg \varphi  \mid \varphi \vee \varphi  \mid \X \varphi  \mid
 \Y \varphi  \mid \varphi \U \varphi \mid \varphi \Since \varphi.
$
Basically, these automata do not need a class automaton.
The construction is equally straightforward for all types of class
formulas. In these cases, basically only class automata are needed.
To deal with the $\delta$-shift in formulas of the form $\C[\delta]{a}
\psi$ we use  the propositions $=_r$. E.g., to validate with respect to
$\psi = \C[7]{a} \CF \chi$ at position $i$, the class automaton of
$\calA'_\psi$ infers from the $=_r$ propositions how many positions the
class word has between $i$ and $i+7$, then it skips these positions
and starts searching for a $\chi$-position from there.
\qed
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "start"
%%% ispell-local-dictionary: "english"
%%% End: 


==> decidabilitycor.tex <==
\subsection{\dataltlx is decidable} \label{sec:multDimDecidable}  


\begin{theorem} \label{theo:ltlmanyd}
  Satisfiability for \classpltl is decidable.
\end{theorem}
  \begin{proof}
    Thanks to Theorem
    \ref{theo:sat1bltl}  it suffices to reduce the satisfiability problem for \dataltl to the
    satisfiability problem for \classpltl on 1-\attwords. That is, for a given \classpltl formula
    $\chi$, we construct a \dataltl formula $\chi'$ such that $\chi'$
    holds for some 1-\attword if and only if $\chi$ holds for some \attword. Therefore we use an encoding of \attwords by 1-\attwords that has been introduced in \cite{DemriLN07}.

    Let $\calP$ and $\calV = \{a_1, \ldots, a_m\}$ be the set of propositions and the set of attributes used in $\chi$, respectively. The set of propositions used in $\chi'$ is $\calP \cup \calV \cup \{R\}$.
  
    The intuition is that every position $i$ of a model $w$ of $\chi$
    is encoded by a block of $m$ positions in a model $w'$ of
    $\chi'$. Position $j$ in the $i$-th block of $w'$ thus represents
    attribute $a_j$ of the $i$th position of $w$. However, as some
    positions in $w$ might not carry values for all
    attributes, the positions corresponding
    to existing attributes are marked by proposition $R$ (see
    Figure \ref{figure:dataltldec} for an example). 
    
    \begin{figure}[t] 
\centering
%\setlength{\arraycolsep}{1.2mm}
\small
	  $ w = 
\begin{array}{|c||c|c|c|}\hline
 \text{Pos} & 1 & 2 & 3 \\\hline
	\text{Props}    & p & q & p,q\\\hline
	    \tatt_1 & d_1 & - & d_3\\
	    \tatt_2 & - & d_2 & d_4\\\hline
	  \end{array}$
\hspace{1cm}
	  $w' = \begin{array}{|c||c|c||c|c||c|c|}\hline
 \text{Pos} & 1 & 2 & 3 & 4 & 5 & 6\\\hline
&	    p & p & q & q & p,q & p,q\\
\text{Props} &	    \tatt_1 & \tatt_2 & \tatt_1 & \tatt_2 & \tatt_1 & \tatt_2\\
	       & R &       &       & R     & R     & R\\\hline
a &	      d_1 & d_2   & d_3   & d_2   & d_3   & d_4\\\hline
	  \end{array}$\\

      \caption{How an \attword $w$ with two attributes is encoded as 1-\attword $w'$. \label{figure:dataltldec}}
    \end{figure}

    The formula $\chi'$ constructed from $\chi$ is of the form
    $\varphi_{\text{structure}}\land t(\chi)$ where
    \begin{itemize}
    \item $\varphi_{\text{structure}}$ makes sure that the 1-\attword
      is well-formed, that is, it is a concatenation of blocks of
      length $m$, where, in each block, the $j$-th position has
      proposition $\tatt_j$ (and no other $\tatt_k$) and all positions
      carry the same propositions from $\calP$, and
    \item $t(\chi)$ is obtained from $\chi$ by a straightforward
      inductive construction.
    \end{itemize}


The translation $t$ makes use of additional translations $t_i$ and
$t_{\max}$. More precisely, 
\[
t_i(\varphi)=\bigvee_{j=1}^m (\tatt_j \ra X^{i-j}\varphi),
\]
and
\[
t_{\max}(\varphi)=\bigvee_{i=1}^m \bigg(\tatt_i \ra
\bigvee_{\delta=0}^{m-i} \big((@a=X^\delta @a \land
\bigwedge_{\delta'=\delta+1}^{m-i} \neg @a=X^{\delta'} @a) \ra \X^\delta\varphi\big)\bigg),
\]
Here, we use $@a=X^\delta @a$ as an abbreviation for $\C[\delta]{a} (R
\land \att a)$.
Intuitively, $t_i(\varphi)$ is a formula which first navigates to
the $i$-th position of the current block and evaluates
$\varphi$. Likewise,  $t_{\max}(\varphi)$ is a formula which first navigates to
the last position of the current block with the same (active) data value  and evaluates
$\varphi$.

    The inductive translation $t$ of positional formulas $\chi$ is defined by
    \begin{itemize}
      \item $t(p) := p$ for all $p \in \calP$
      \item $t(\neg \varphi) := \neg t(\varphi)$
      \item $t(\varphi \vee \psi) := t(\varphi) \vee t(\psi)$

      \item $t(\X \varphi) := \X^m t(\varphi)$
      \item $t(\varphi \U \psi) := t(\varphi) \U t(\psi)$

      \item $t(\att a_i = \X^k \att  a_j) := t_{i}(\att
        a=X^{km+(j-i)}\att a)$

      \item $t(\C{a_i} \varphi) := t_i(R \land t(\varphi))$
    \end{itemize}	
    for all $i, j \in \{1, \ldots, m\}$. Translations of the positional formulas for the past are analogous.

    Now we give the translation for class formulas. Here, the basic
    idea is that each navigation step ends at a position with
    the currently frozen data value. 
      \begin{itemize} 
      \item $t(\att a_j) := \bigvee_{i=1}^m(\tatt_i \rightarrow (\att
        a=X^{j-i}\att a))$
      \item $t(\neg \varphi) = \neg t(\varphi)$
      \item $t(\varphi \vee \psi) = t(\varphi) \vee t(\psi)$
      \item $t(\CX \varphi) = t_{\max}(\CX(\neg R \CU (R \wedge t(\varphi))))$
      \item $t(\varphi \CU \psi) = (R \rightarrow t(\varphi)) \CU (R \wedge t(\psi))$
    \end{itemize}
    The translations for the past operators are analogous. The
    correctness of the reduction is straightforward.

\qed \end{proof}
The complexity of the satisfiability problem for \dataltl over
1-\attwords is probably very bad. As for two-variable logics \cite{BojanczykMSSD2006}, it is
(efficiently) interreducible with the reachability problem for Petri
Nets \cite{EsparzaN94}.  

%A proof sketch is given in the appendix.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "start"
%%% ispell-local-dictionary: "english"
%%% End: 


==> decidabilityinf.tex <==
\subsection{$\classpltl$ on infinite \attwords is decidable} \label{sec:infdecidable}
Over attributed $\omega$-words \classpltl remains decidable. First, we
observe that the mapping used in Theorem \ref{theo:ltlmanyd} works
also for the infinite case, i.e. the satisfiability problem for
\dataltl over attributed $\omega$- words is reducible to the
satisfiability problem over 1-attributed $\omega$-words. Hence, it remains to prove the decidability for the latter problem. We do this by a reduction to the non-emptiness problem for data $\omega$-automata which is shown to be decidable in \cite{BojanczykMSSD2006}.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
These automata are defined analogously to data automata.
We only describe the differences here. A data $\omega$-automaton
$\aut{A} = \dataautinf{\baseautinf{B}}{\classaut{C}}{\classautinf{C}}$
consists of a base automaton $\baseautinf{B}$ which is a Büchi
letter-to-letter transducer with output over some alphabet $\Gamma$, a
finitary class automaton $\classaut{C}$ which is a finite string
automaton over $\Gamma$ and an infinitary class automaton
$\classautinf{C}$, which is another Büchi automaton over $\Gamma$. An
1-attributed $\omega$-word $w$ is accepted if the base automaton has
an accepting run over the string projection of $w$ with output
$\gamma_1\gamma_2 \ldots$ such that for every finite class $i_1 <
\ldots < i_m$ the string $\gamma_{i_1} \ldots \gamma_{i_m}$ is
accepted by $\baseaut{B}$ and for every infinite class $i_1 < i_2 <
\ldots$, the $\omega$-string $\gamma_{i_1}\gamma_{i_2} \ldots$ is accepted by 
$\baseautinf{B}$.

\begin{theorem} \label{theo:satinfdataltl}
Satisfiability for \dataltl on attributed $\omega$-words 
is decidable.
\end{theorem}  

\begin{proof} (Sketch)
The proof is by reduction to the non-emptines problem for data
$\omega$-automata and is along very similar lines as that of Theorems
\ref{theo:sat1bltl} and \ref{theo:ltlmanyd}. By applying the mapping
given in Theorem \ref{theo:ltlmanyd} we first make a reduction to the
satisfiability problem for \dataltl on 1-attributed $\omega$-words. Then, given a \dataltl formula $\varphi$ defined on $\{a\}$-complete \attwords we can construct a data $\omega$-automaton which is non-empty if and only if $\varphi$ is satisfiable. 
%As Lemma \ref{theo:ltlmanyd} holds also for $\omega$-automata  it is sufficient to construct an automaton $\aut{A} = \dataautinf{\baseautinf{B}}{\classaut{C}}{\classautinf{C}}$ that reads correctly $k$-marked attributed $\omega$-words. 
The automaton $\calA_\psi'$ that checks whether a given word is valid with respect to a formula $\psi$ differs from its counterpart in the finite case, basically, only for $\psi = \varphi_1 \U \varphi_2$ or 
$\psi = \varphi_1 \CU \varphi_2$. The difficulty is to ensure that whenever $\psi$ occurs the formula 
$\varphi_2$ definitely occurs in future. But these cases can be
handled easily using classical techniques in automata construction for
temporal logics on $\omega$-words \cite{VardiW94}. For a formula $\psi
= \varphi_1 \U \varphi_2$ the automaton $\calA_\psi'$ checks that the
input word has a suffix where either positions labeled with $\psi_1 \U
\varphi_2$ and $\varphi_2$ or positions labeled with $\neg(\varphi_1 \U \varphi_2)$ occur infinitely often.
The acceptance condition for the class operator $\CU$ is defined
analogously. \qed
\end{proof}

==> definitions.tex <==
\section{Definitions} \label{sec: def}
We first fix the data model and define \dataltl afterwards. Finally we
give an example that illustrates the way in which properties can be
expressed 
 \subsection{Attributed words} \label{baseDef}
 Let $\Prop$ and $\Att$ be (possibly infinite) sets of propositions and attributes and $\D$ an infinite set of data values. 
An \textit{\attword} $w$ is a finite word where every position carries
a finite set $\{p_1, \ldots, p_l\}$  of propositions from $\Prop$ and
a finite set $\{(a_1,d_1),\ldots,(a_k,d_k)\mid \text{ $a_i \neq a_j$ for $i \neq j$}\}$ of attribute-value pairs
from $\Att\times\D$.
  
 Given an \attword $w$ we denote the proposition set of position $i$
 in $w$ by \labeling{w}{i}. 
A position $i$ is a
\emph{$p$-position} if $p\in\labeling{w}{i}$. 
%This set will also be called the
                            %\textit{label} of $i$. 
By $\mdata{w}{a}{i}$ we denote the value of attribute $a$ on position
$i$. If position $i$ does not carry attribute $a$, then
$\mdata{w}{a}{i} = \nil \notin D$. The \textit{word projection} of an
\attword $w = w_1 \ldots w_n$ is defined by $\stringpr{w}
:= \labeling{w}{1} \ldots \labeling{w}{n}$. 
By $\pos{w}{d}$ we denote the set of \textit{class positions} of $d$
in $w$, that is,  the set of positions of $w$ with at least
one attribute with value $d$. 
The \textit{class word} $\class{w}{d}$ of $w$ with respect to $d$ is
the restriction of $w$ to the positions of $\pos{w}{d}$. 

We always consider sets of words over some finite set $\calP$ of
propositions and a finite set $\calV$ of attributes\footnote{As we
  will use $\calA$ for automata we use $\calV$ here: {\bf V}ariables.}. We call an
\attword $w$ \emph{$\calV$-complete} for a finite set $\calV\subs\Att$ if
every position of $w$ has exactly one pair $(a,d_a)$ for each
$a\in\calV$. A $\{a\}$-complete word is called
\emph{1-\attword}. We refer to the value of attribute $\att a$ at a
position $i$ in a
1-\attword as \emph{the data value of $i$}.
There is an immediate correspondence between
data strings (that is, sequences of (symbol,value) pairs) and
1-\attwords. Thus, we use in this paper automata and logics that were introduced
for data strings also for 1-\attwords.

Attributed $\omega$-words are defined accordingly.

%We will also consider \text{\datastrings} which are special \attwords where every position carries %exactly one attribute $a$. Sometimes we simply will call \attwords \textit{words} and %\datastrings  \textit{strings}.  

For $i, j \in \N$ with $i \leq j$ we denote the interval $\{ i, i+1,
\ldots j \ \}$ by $[i, j]$. As usual we use round brackets to denote
open intervals, e.g., $[3,5)=\{3,4\}$.


\subsection{\dataltlx}
The logic \dataltlx (abbreviated: \dataltl) has two main types of formulas, \textit{position
  formulas} and \textit{class formulas}, where, intuitively, class formulas
express properties of class words. We first state the syntax of the
logic and give an intuitive explanation of its non-standard features afterwards.

  %It is possible to test whether an attribute has data value $d$. Positional formulas are LTL-formula that allow for moving in the whole \attword. 
We fix a finite set $\calP \subseteq \Prop$ of propositions and a
finite set $\calV \subseteq \Att$ of attributes.

The syntax of \emph{position formulas} $\varphi$ and \emph{class formulas}
$\psi$ of \dataltl (over $\calP$ and $\calV$) are
defined as follows.
\begin{eqnarray*}
  \varphi  &::=& p \mid \neg \varphi  \mid \varphi \vee \varphi  \mid \X
  \varphi  \mid \Y \varphi  \mid \varphi \U \varphi \mid \varphi
  \Since \varphi \mid \C[\delta]{a} \psi\\
\psi &::=& \varphi \mid\att{a} \mid \neg \psi \mid \psi \vee \psi \mid  \CX \psi \mid \CY \psi \mid \psi \CU \psi \mid \psi \CS \psi
\end{eqnarray*}

Here, $p \in \calP$, $a\in \calV$, $\delta \in \Z$.
Intuitively, the quantifier $\C{a} \psi$ restricts the evaluation of
$\psi$ to the class word induced by attribute $a$ at the current
position.


Next we define the formal semantics of position formulas. Let $w$ be an \attword and $i$ a position on $w$:  
\begin{itemize}
    \item $w,i \models p$ if $p \in \labeling{w}{i}$;
    \item $w,i \models \neg \varphi$ if $w,i \not\models \varphi$;
    \item $w,i \models \varphi_1 \vee \varphi_2$ if $w,i \models \varphi_1$ or  $w,i \models \varphi_2$;
    \item $w,i \models \X \varphi$ if $i+1 \leq |w|$ and $w,i+1 \models \varphi$;
    \item $w,i \models \varphi_1 \U \varphi_2$ if there exists a $j \geq i$ such that $w,j \models \varphi_2$ and $w,j' \models \varphi_1$ for all $j' \in [i,j)$;
    \item $w,i \models \C[\delta]{a} \psi$ if $\mdata{w}{a}{i} \neq
      \nil$, $i+\delta\in[1,|w|]$, and $w,i+\delta, \mdata{w}{a}{i} \models \psi$.
  \end{itemize}
The operators  $\Y$ and $\Since$ are the past counterparts of $\X$ and
$\U$ respectively. Their semantics is defined analogously\footnote{To
  avoid ambiguity:   $p\Since q$ holds if there is a $q$-position in
  the past and at the intermediate positions $p$ holds.}.


Next, we define the semantics of class formulas. Let $w$ be an \attword, $i$ a position on $w$ and $d$ a data value.
\begin{itemize}
    \item $w, i, d \models \varphi$ if $w,i \models \varphi$;
\item $w,i,d \models \att a$ if $\mdata{w}{a}{i} = d$;
%    \item $w, i, d \models \att a$ if $\mdata{w}{a}{i} = d$
%    \item $w, i, d \models \neg \varphi$ if $w, i, d \not\models \varphi$
 %   \item $w, i, d \models \varphi_1 \vee \varphi_2$ if $w, i, d \models \varphi_1$ or $w, i, d \models \varphi_2$
    \item $w, i, d \models \CX \varphi$ if there exists a  $j \in
      \pos{w}{d}$ with $j > i$, and for the smallest such $j$ it holds  $w, j, d \models \varphi$;
    \item $w, i, d \models \varphi_1 \CU \varphi_2$ if there exists a
      $j \in \pos{w}{d}$ with $j \geq i$ such that $w,j,d \models
      \varphi_2$ and $w,k,d \models \varphi_1$ for all $k \in
      \pos{w}{d}\cap[i,j)$. 
  \end{itemize}
 
  For  the past class operators $\Y$ and $\Since$ the semantics is defined
  analogously and the semantics of the Boolean connectors is as usual. Finally,  $w\models\varphi$, if $w, 1 \models
  \varphi$. 
We denote the set of positional formulas by \dataltl. 

Besides $\bot$ and $\top$ we use the following usual abbreviations:
\begin{center}
\begin{tabular}[h]{cccc} 
$\F \varphi : = \top \U \varphi $ & $\G \varphi := \neg \F \neg \varphi$ & $\Past \varphi : = \top \Since \varphi $ & $\Hist \varphi := \neg \Past \neg \varphi$
\end{tabular}
\end{center} 
The abbreviations $\CF$ and $\CG$
and their past counterparts are defined analogously. Furthermore, 
we abbreviate $\C[\delta]{a} \att b$ by $\kXT{\delta}{a}{b}$. 

%The set of all \attwords satisfying a formula $\varphi$ is denoted by $\calL(\varphi)$.

\ignore{
 \subsection{Examples} \label{sec:express}
  
  We provide some examples to illustrate the expressive power of \dataltl.

  \begin{example}{Example properties}
    \begin{itemize}
      \item [a)] '$\varphi$ holds at the next position that carries the same data value on attribute $b$ as the current position carries on attribute $a$' can be expressed by $\C{a}(\CF \rightarrow (\neg \att{b} \CU (\att{b} \wedge \varphi)))$. 
      \ahmet{Zu der informellen Beschreibung würde doch eher die Formel 
      $C_a(\CF b \rightarrow (\neg b \CU (b \wedge \varphi)))$ passen.}
      \item [b)] If attribute $b$ is present at all positions, i.e. $\G \C{b} \top$, then  '$\varphi$ holds at the next position that carries another data value on attribute $b$ than the current position carries on attribute $a$' can be expressed by 
      $(\neg \kXT{1}{a}{b} \wedge \X \varphi) \vee \X( \kXT{1}{b}{b} \U (\neg \kXT{1}{b}{b}  \wedge \X \varphi))$.

    \end{itemize}
  \end{example}
}

\subsection{Example: a simple client/server scenario}
The following example illustrates how properties can be expressed in \dataltl.

 % \begin{example}{Client/Server}
    Consider an internet platform that uses $m$ servers $S_1, \ldots,
    S_m$ to process queries from clients. Every client shall have a
    unique client number. As we do not know beforehand how many
    clients will use the platform, we model the client numbers by the set $\D=\mathbb{N}$.

    Each of the servers can either idle, be queried by a client or serve the answer for a query. For server $j$,  the actions are modelled by the set of propositions $\{q_j,s_j,i_j\}$. Runs of the internet platform can now be represented by an \attword with attribute set $\Att = \{S_1, \ldots, S_m\}$ and set of propositions $\bigcup_{1 \leq j \leq m} \{q_j,s_j,i_j\}$. That a server $S_j$ shall perform exactly one action from $\{q_j, s_j, i_j\}$  at any given time, can be easily expressed by a \dataltl-formula.

    Let us look at an example system with three servers $A$, $B$ and
    $C$. An example run represented as an \attword could look as follows.    
{\small
    $$\begin{array}{|c|*{6}{|c}|}\hline
\text{Pos} & 1 & 2 & 3 & 4 & 5 & 6 \\\hline
	 \text{Props}   & \{q_A,q_B,i_C\} & \{q_A,q_B,q_C\} & \{s_A,q_B,s_C\} & \{s_A,s_B,i_C\} & \{i_A,s_B,q_C\} & \{i_A,s_B,s_C\} \\\hline
	A & 1 & 2 & 2 & 1 & - & - \\
	B & 2 & 3 & 4 & 2 & 3 & 4\\
	C & - & 1 & 1 & - & 2 & 2\\\hline
      \end{array}$$
 }   Here, e.g., at position $5$ server $A$ is idling, server $B$ is serving client 3 and server $C$ is queried by client 2.
    Properties of runs can be expressed by \dataltl formulas:
      \begin{itemize}
	\item A client can query a second time on a server only after the first query has been served:
	  $$\bigwedge_{Z \in \{A,B,C\}}\G(q_Z \rightarrow \C{Z}((\att{Z} \rightarrow \neg q_Z)\CU(\att{Z} \wedge s_Z)))$$
	\item A server $Z$ can serve a client only if there is an unanswered query by that client (i.e.~the last action by that client on $Z$ was a query):
	  $$\bigwedge_{Z \in \{A,B,C\}}\G(s_Z \rightarrow \C{Z}((\neg \att{Z}) \CS(\att{Z} \wedge q_Z))))$$
	\item A client with an open query on server $A$ shall only be allowed to query server $C$ until server $A$ answered the query:
$$ G( q_A \rightarrow \C{A}(\neg \att{B} \wedge \CX(( \neg (q_A \wedge A) \wedge \neg (q_B \wedge B)) \CU  s_A)))$$
      \end{itemize}
%  \end{example}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "start"
%%% ispell-local-dictionary: "english"
%%% End: 


==> expressiveness.tex <==

\section{Expressiveness of \dataltl} \label{sec:discussion}
  In this section we will give a short overview of established logics
  on strings with data values and outline how \dataltl fits in. 
%Furthermore we sketch a couple of variations of \dataltl and explain why we choose the given %definition.
 We give a short introduction to freeze LTL and $\text{CLTL}^\diamond$, see \cite{DemriLazicLTL09} and \cite{DemriSG2007} for more details. Afterwards we compare these two logics to \dataltl.

\subsection{\dataltl versus \freezeLTL}
 \textit{Freeze LTL} is an extension of \LTL for data words by a freeze quantifier
  that binds the data value of the current position to a variable (aka
  register) and allows to compare the value of a position with the
  value bound to a variable. Satisfiability for freeze \LTL is
  undecidable even for two registers \cite{DemriLazicLTL09},
  therefore \cite{DemriLazicLTL09}  proposed the 1-register fragment
  \freezeLTL.
In the framework of 1-\attwords,  formulas of \freezeLTL are of the form
    $$\varphi ::=  p \mid \store \varphi \mid \fetch \mid \neg \varphi \mid \varphi \wedge \varphi \mid \X \varphi \mid \Y \varphi \mid \varphi \U \varphi \mid \varphi \Since \varphi.$$
The formal semantics of \freezeLTL (on data strings) can be found in
\cite{DemriLazicLTL09}. We illustrate it by a simple example: the
formula $\G (p\to (\store \F (q \land {\fetch})))$ expresses that each
$p$-position has a future $q$-position with the same data value.   
  
In \cite{DemriLazicLTL09}, the fragment simple \freezeLTL was
invented,  where at most one temporal operator is allowed between the
the freeze quantifier $\store$ and a value test $\fetch$. Furthermore,
only the unary temporal operators $\X^k, \Y^{k}, \X^k\F, \Y^{k}\Past$,
$k\in \N$ are allowed. Here, $\X^k\F$ is considered a single operator,
that is $\store\X^k\F{\fetch}$ is an allowed formula.
%  
The relative expressive power of \dataltl and \freezeLTL can be
summarized in the following two propositions.
\begin{proposition}
  Every property of 1-\attwords that is expressible in \dataltl can also be expressed in \freezeLTL.
\end{proposition}
The statement also holds for all extensions of \dataltl considered in
Section \ref{sec:extended}. Note however, that \freezeLTL is undecidable whereas
\dataltl and its main extension in Section \ref{sec:extended} are decidable.

 \begin{proposition}\label{prop:simple}
    The following logics are equivalent on 1-\attwords
    \begin{itemize}
      \item [(i)] Simple \freezeLTL
      \item [(ii)] \dataltl without Until and Since extended
        by $\F^\delta_{\not=}$ and $\Past^\delta_{\not=}$.
    \end{itemize}
  \end{proposition}
Here, $\F^\delta_{\not=}\varphi$  intuitively navigates to a future position
of distance $\ge \delta$ with a different data value and evaluates
$\varphi$ there. In the notation
of Section \ref{sec:extended} it is an abbreviation for $\top
\Uattd{a} (\notdata{a} \land \varphi)$. Note, that an analogous operator $F^\delta_= \varphi$ for equal data values can be simulated by $\C[\delta]{a} F^= \varphi$. The proof of both propositions
is straightforward and therefore omitted.

% For example a class formula $\C{a} \varphi$ can be simulated by storing the current data value in the register and moving along the word considering only positions that satisfy $\fetch$. \freezeLTL is even more expressive than \dataltl as the formula  $p \wedge \store \F(q  \wedge \F (r \wedge \fetch))$ can not be expressed in \dataltl. This is because being able to express this property would yield undecidability of the satisfiability problem (see Section \ref{sec:undecidability}). %Nevertheless, some properties, as for example $\store \F (q \wedge (\fetch \rightarrow r) \U (\fetch \wedge s))$, can be translated to \dataltl.  
    

% Whereas the future fragment of \freezeLTL is decidable\footnote{Here and
%   henceforth a logic is called \emph{satisfiable} if its
%   satisfiability problem over (1-)\attwords is decidable.} \cite{DemriLazicLTL09}, \freezeLTL was shown to be undecidable even if only the operators $\Past$ and $\F$ are used \cite{FigueiraS2009}. As opposed to this, finite satisfiability for \dataltl is decidable (see Section \ref{sec:decidability}).
%     \freezeLTL restricted to the future operators is decidable and strictly captures the future fragment of \dataltl for 1-valued data strings. Yet \dataltl remains decidable even when using more than one attribute. 

    
%     The operators  $\U$, $\X^=$ and $\U^=$ are not expressible in simple \freezeLTL, but every simple \freezeLTL formula can be translated to an equivalent \dataltl formula on $1$-valued data strings:
    
 %  \thomasZ{Modify operators as soon as the definitions section is stable.}
%   \thomasZ{Definition of $FO^2$ and the proof of the Lemma for the appendix can be found in the sources. (Has to be adapted as soon as the definitions section is stable.)}
 
  % appendix

\subsection{\dataltl versus $\text{CLTL}^\diamond$} 

  \textit{Temporal logic of repeating values ($\text{CLTL}^\diamond$)} was introduced in \cite{DemriSG2007}. $\text{CLTL}^\diamond$-formulas are of the form
    $\varphi ::=  x = X^\delta y \mid x = \diamond y \mid \varphi \wedge \varphi \mid \neg \varphi \mid \X \varphi \mid \varphi \U \varphi \mid \Y \varphi \mid \varphi \Since \varphi$,
  where $x,y$ are from a set of variables. A CLTL$^\diamond$-formula with variables $\{x_1, \ldots, x_m\}$ is evaluated on
  sequences of $m$-tuples of data values (without labels from a finite set) but the extension to   
  $\{x_1, \ldots, x_m\}$-complete attributed strings is straightforward. 
  A formula $x = X^\delta y$ tests whether component $x$ of the
  current position has the same data value as component $y$ of the
  $\delta$-next position. A formula $x = \diamond y$ is true if there
  is a (strict) future position with the same data value on component $y$ as
  the current position has on component $x$. The semantics of all
  other operators is as usual. 

The following proposition is straightforward, since $x = \diamond y$ and $x = X^\delta y$ can be encoded by $\C[0]{x}  \CX \CF \att{y}$ and $\C[\delta]{x} \att{y}$, respectively.
  \begin{proposition}
    On $\{x_1, \ldots, x_m\}$-complete \attwords
    \classpltl is strictly more expressive than $\text{CLTL}^\diamond$.
  \end{proposition}
%   \thomasZ{Even decidability of infinite satisfiability of CLTL$^\diamond$ was proved. Modify if we also proof the infinite case.}
%   Finite satisfiability CLTL$^\diamond$ was shown to be decidable in \cite{DemriSG2007}. For $m$-valued data strings \dataltl captures CLTL$^\diamond$. However, \dataltl is much more expressive because not only the existence of a future position with the same data value can be tested, but also a formula can be evaluated at that future position. Thus: 

% % \thomasZ{The proof of the Lemma for the appendix can be found in the sources. (Has to be adapted as soon as the definitions section is stable.)}
%   \begin{lemma}
%     \classpltl on $m$-valued data strings is strictly more expressive than $\text{CLTL}^\diamond$.
% %     \begin{proof}
% %       Let $\varphi$ be a CLTL$^\diamond$-formula with variables $\{x_1, \ldots, x_m\}$. We define a \dataltl formula $\psi = \psi_\text{att} \wedge \psi_\varphi$ that uses the attributes $\Att = \{x_1, \ldots, x_m\}$ and has the same models as $\varphi$.
% % 
% %       Firstly, $\psi_\text{att}$ ensures that all attributes occur on every position by conjuncting $\G(\C{x} \top)$ for all attributes $x$. $\psi_\varphi$ is an inductive translation of $\varphi$. Formulas of the form $x = \diamond y$  are mapped to $\C{x}(\CF y)$. All other translations are straightforward.
% %     \end{proof}
%   \end{lemma}
 
\ignore{
  \subsection{Design decisions.}
  \thomasS{Diese beiden würde ich eher im Vergleichskapitel diskutieren:
\begin{tabular}[h]{c}
$\Xbar[\delta]{a} \varphi:= \C[\delta]{a}( \varphi_{\text{skip}}\CU (\varphi_{\text{skip}} \wedge \bigvee_{a,b \in \calV} (\neg \kXT{1}{b}{c}) \wedge \X  \varphi ) )$ 
\end{tabular}
\begin{tabular}[h]{c}
$\Ybar[\delta]{a} \varphi:= \C[\delta]{a}( \varphi_{\text{skip}}\CS (\varphi_{\text{skip}} \wedge \bigvee_{b,c \in \calV} (\neg \kXT{-1}{b}{c}) \wedge \Y  \varphi ) )$ 
\end{tabular}

where $\varphi_{\text{skip}} = \bigwedge_{b \in \calV}(\C{b} \top
\rightarrow \att b)$.  Intuitively, $\Xbar[\delta]{a} \varphi$ first jumps $\delta$ forward, then jumps to the first position carrying at least one different attribute value than the value of attribute $a$ of the starting position and tests $\varphi$.  
}
  \thomasZ{This section has still to be done properly.}
  
  \thomasZ{Reasoning is not really good.}
   \thomasZ{Being on a position with an attribute $a$ that has data value $d$, the $\C{a}$-operator allows for moving along all positions that have at least one attribute $b$ with data value $d$. A slight extension of the $\C{a}$-operator to more attributes already yields undecidability.}
 


  \textit{Choice of Operators.} Data LTL offers usual navigation on the whole word as well as navigation along certain data values. This can be implemented in formulas in two ways. First, as \dataltl does, by using a two-level approach comparable to CTL. Second, by using usual LTL operators as well as operators for moving along certain data values. For example the operator $X^=_{\att{a}} \varphi$ could say 'move to the next position with an attribute that has a data value equal to the data value at attribute $a$ of the current position'. However, this notation becomes awkward, when defining an operator for $\C[\delta]{a}{(X^{=} \varphi)}$. Thus for notational reasons we choose to separate global movements and movements along one data value. 

  Intuitively, the $\U$-operator $\varphi \dataU \psi$ allows for testing $\varphi$ along positions with one equal data value until $\psi$ is fulfilled on a position with an equal data value. On the other hand, $\varphi \Ubar \psi$ allows for testing $\varphi$ on positions with arbitrary data values or positions with different data values until $\psi$ is fulfilled on a position with a different data value. This leaves room for $\U$-operators $\varphi \DUe \psi$ and $\varphi \DUue \psi$, that test $\varphi$ on positions with arbitrary data values and on positions positions with different data values, respective, until $\psi$ is fulfilled at a position with an equal data value. However, in Section \label{sec:undecidability} we show that these operators lead to undecidability.

\textit{Semantics of the Class Operator $\C{a}$.}
 $\C{a}$ restricts the string to positions where there is at least one attribute with the same data value as the current value of $\att{a}$. The following alternatives could have been considered:
\begin{itemize}
  \item An operator $\Ca{a}$, that restricts to positions where the attribute $a$ carries the same data value as the current value of $\att{a}$.
  \item An operator $\Cb{a}$, that restricts to positions where all attributes carry the same data value as the current value of $\att{a}$.
\end{itemize}
However, $\Ca{a} \varphi$ can be simulated by the $\C{a}$-operator by substituting every subformula $\psi$ of $\varphi$ that is in the scope of $\Ca{a}$ by $\att{a} \wedge \psi$. Similarly $\Cb{a} \varphi$ can be simulated by substituting every subformula $\psi$ of $\varphi$ that is in the scope of $\Ca{a}$ by $(\bigwedge_{a \in \Att} \C{a} \top \rightarrow \att{a}) \rightarrow \psi$. As $\C{a}$ can also demand that only positions with attribute $a$ and $b$ with equal data value will be considered, $\C{a}$ is more general then both $\Ca{a}$ and $\Cb{a}$.

\subsection{Attributes vs.~Multi-Valued Data Words.}

\dataltl formulas use \attwords as models, that is every position carries a subset $S$ of the set of attributes $\Att$ as attributes. An alternative is to use $m$-valued data words as models. Both approaches are equivalent. An $m$-valued data word can be simulated by an \attword that carries $m$ attributes on all positions. \attwords with $m$ attributes can be simulated by an $m$-valued data word with an additional proposition $p_i$ for every attribute $a_i$ that marks the positions where attribute $a_i$ is present.

\ahmet{Auch auf Propositionen versus Alphabet eingehen}




%The main goal of \dataltl is to allow LTL-like movements on data classes. When only one attribute is available then there is only the possibility to move along equal data values of , then it is straight-forward to use operators that can move to the next position with an equal data value as the current position. Similarly for an Until-Operator on data values. For more than one attribute 
% \example{Example properties}{
%     \begin{itemize}
%       \item [a)] '$\varphi$ holds at the next position that carries the same data value on attribute $b$ as the current position carries on attribute $a$' can be expressed by $\C{a}(\CF \rightarrow \CX(\neg \att{b} \CU (\att{b} \wedge \varphi)))$. 
%       \ahmet{Zu der informellen Beschreibung würde doch eher die Formel 
%       $C_a(\CF b \rightarrow (\neg b \CU (b \wedge \varphi)))$ passen.}
%       \item [b)] If attribute $b$ is present at all positions, i.e. $\G \C{b} \top$, then  '$\varphi$ holds at the next position that carries another data value on attribute $b$ than the current position carries on attribute $a$' can be expressed by 
%       $(\neg \kXT{1}{a}{b} \wedge \X \varphi) \vee \X( \kXT{1}{b}{b} \U ( \kXT{1}{b}{b}  \wedge \X \varphi))$.
% 
%     \end{itemize}
%   }
}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "start"
%%% ispell-local-dictionary: "english"
%%% End: 

==> intro.tex <==
\section{Introduction}

Motivated by questions from XML theory and automated verification, extensions of (finite or infinite) strings by
data values from unbounded domains have been studied intensely in
recent years. Various
logics and automata for such data words have been invented and
investigated. 

A very early study by Kaminski and Francez
\cite{KaminskiF94} considered 
automata on strings over an ``infinite alphabet''. In
\cite{Bouyer02}, \emph{data words} were invented as finite 
sequences of pairs $(\sigma,d)$, where $\sigma$ is a symbol from a
finite alphabet and $d$ a value from a possibly infinite domain. In
\cite{BouajjaniHJS07}  multi-dimensional data words were
considered where every position carries $N$ variable valuations, for
some fixed $N$. Similar models can be found for instance in \cite{AronsPRXZ01} and other work
on parameterized verification. More powerful models were investigated
in \cite{LisitsaP05} and \cite{DeutschHull+Automatic09} where every position is
labeled by the state of a relational database, i.e., by a set of relations over a
fixed signature. 

For the basic model of data strings with one data value per position
a couple of automata models and logics have been invented and
their algorithmic and expressive properties have been studied. On the
automata side we mention register automata \cite{KaminskiF94,BouyerPTalgebraic03,NevenSV04}
(named \emph{finite memory automata} in \cite{KaminskiF94,BouyerPTalgebraic03}), pebble
  automata \cite{NevenSV04,Tan09}, alternating 1-register automata
  \cite{DemriLazicLTL09}, data automata \cite{BojanczykMSSD2006} (or
  the equivalent class memory automata \cite{BjorklundS10}).

On the logical side, classical logics like two-variable first-order
logic \cite{BojanczykMSSD2006} have been studied and recently order
comparisons between data values have been considered
\cite{Manuel10,SchwentickZ10}. The satisfiability problem for  two-variable first-order
logic over data words is decidable if data values can only be compared for equality
but positions can be compared with respect to the linear order and the
successor relation \cite{BojanczykMSSD2006}. However, the complexity
is unknown. It is elementary if and only if testing
reachability in Petri nets is elementary as well \cite{BojanczykMSSD2006}. The proof of decidability uses \emph{data
  automata}, a strong automata model with decidable non-emptiness. 

More relevant for this paper are
previous investigations of temporal logics on data words. A pioneering
contribution was by Demri and Lazic
\cite{DemriLazicLTL09}  (the journal version
of \cite{DemriL06}) which introduced \frltl. In a nutshell, \frltl extends \LTL by
\emph{freeze quantifiers} which\footnote{We note that the freeze
  quantifier itself was used  already in \cite{Demri04} and in
  previous work, e.g., in \cite{AlurH94}.} allow to ``store'' the current data
value in a register and to test at a possibly different position
whether that position carries the same value. \frltl has a decidable
finite satisfiability problem if it is restricted to one register
(\freezeLTL) and to
future navigation, but the complexity is not primitive recursive. With
one register and past (and future) navigation it is undecidable. In
\cite{FigueiraS2009} it is shown that these lower bounds even hold if
only navigation with $\F$ and $\Past$ (but without $\X$) are allowed. 

In \cite{DemriLazicLTL09}, also a restriction of \freezeLTL,
\emph{simple \freezeLTL}, was investigated and it was shown that it is 
expressively equivalent to two-variable logics. The restriction
requires that (syntactically) between each value test and the corresponding freeze
quantifier there is at most one temporal operator and it disallows Until
and Since navigation but allows past navigation. Thanks to the (effective) equivalence to
two-variable logics, simple \freezeLTL is decidable. 

One of our aims in this paper was to find a decidable temporal logic
on data words with past navigation that is more expressive than simple
\freezeLTL. In particular it should allow Until navigation with reference
to data values. On the other hand, the logics we study are semantical fragments of 
\freezeLTL. Furthermore this work was motivated by the decidable
logic \diamondLTL for multi-attribute data words \cite{DemriSG2007}. It
allows to test whether somewhere in the future (or past) a current
data value occurs and it can compare data values between two positions of
bounded distance. The logics proposed in this paper are intended 
to have more expressive power than  \diamondLTL while retaining its
decidability. 


\paragraph*{Contribution}
 We propose and investigate temporal logics for
 multi-attribute data words. An \attword 
is a string which can have a finite number of (attribute,value)-pairs
at each position (in the spirit of XML) and has propositions
rather than symbols (in the spirit of \LTL).

We first define  \dataltlx which mimics the navigation abilities of simple
\freezeLTL, if only positive register tests are used. As  sequences of
such navigation steps do not do any harm we drop the requirement to
freeze the data value at every step and replace freeze quantifiers by a class
quantifier which restricts a sub-formula to the positions at which
this data value appears.  We show that a slight extension of this
logic captures simple \freezeLTL (Proposition \ref{prop:simple}) and
that it is decidable (Theorem \ref{theo:ltlmanyd}). Although strictly more expressive than \diamondLTL, the decidability proof for \dataltlx is conceptually simpler than the proof given in \cite{DemriSG2007}. It uses an
encoding of multi-attribute words by data words and a reduction to
non-emptiness of data automata. A similar multi-attribute encoding has already been used in \cite{DemriLN07}. The result generalizes to
attributed $\omega$-words (Theorem \ref{theo:satinfdataltl}).
Some obvious extensions (by navigation with respect to two data values or
Until navigation where intermediate positions can be tested by
data-free formulas) are undecidable (Theorems \ref{theo:multi-undec}
and \ref{theo:undU}, respectively). 

Finally, we add a powerful Until-operator to \dataltlx, which allows to
navigate to a position with a data value that is \emph{different} from
the value of a given attribute at the starting
position. Furthermore, it can test properties of intermediate
positions by arbitrary sub-formulas and can even test (in a limited
way) whether
intermediate positions have  attribute values different from or equal
to the value on the starting position. The resulting logic can express all properties expessible in two-variable first-order logic and  contains the Until operator. That this logic is still decidable is the main technical contribution of the paper.


%\paragraph*{Organization}
The paper is organized as follows. In Section \ref{sec: def}, we
define \attwords and \tinm{Basic} \tinm{Data LTL} and give
some example properties. In Section \ref{sec:discussion}, we compare
\dataltlx with other logics.
% and discuss some of our design decisions. 
Section \ref{sec:decidability} shows that \dataltlx is
decidable and presents undecidability results for some
extensions. Section \ref{sec:extended} introduces the extended Until
operator and shows decidability of the resulting logic. It also shows
(the simple fact) that an Until-operator that navigates with respect
to equality and allows (only) data-free intermediate tests quickly
leads to an undecidable logic. We conclude in Section
\ref{sec:conclusion}.


\paragraph*{Related work} We discussed many related papers above.
Another approach, combining temporal and classical  logics, was studied in
\cite{DeutschHull+Automatic09}. It allows to navigate by temporal
operators and to evaluate first-order formulas in states. Properties
depending on values at different states can be stated by  global
universal quantification of values. In \cite{BouajjaniHJS07} a
first-order logic on multi-dimensional data words was studied.

\paragraph*{Acknowledgements}

The idea to extend the temporal logic that is equivalent to
two-variable logics by Until operators (without reference to data)
goes back to a suggestion by Miko{\l}aj Bojanczyk \cite{Bojanczyk06}.
We are also indebted to Volker Weber with whom we carried out first
investigations before he tragically passed away in 2009.
The remarks by the reviewers of FSTTCS 2010 helped to improve the
presentation and to add some additional references.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "start"
%%% ispell-local-dictionary: "english"
%%% End: 


==> undecidability.tex <==
\subsection{Undecidable Extensions} \label{sec:undecidability}
Extensions of \dataltl quickly yield undecidability. We consider two
such extensions here. 
%The proofs of the following two results are given in the appendix.

\paragraph*{\dataltl with Navigation along Tuples} \label{sec:tuplecomp}

We extend $\C{a}$ to a quantifier $\multiC{a}{b}$ that `freezes' the values $d_a$ and $d_b$ of the attributes $a$ and $b$, respectively. Operators $\CX, \CY, \CU$ and $\CS$ in the scope of $\multiC{a}{b}$ then move along positions that have attributes with data values $d_a$ and $d_b$. At such positions the values of tuples of attributes can be tested for equality with $(d_a,d_b)$. For example the property `there is a future position with proposition $p$ where attribute $c$ carries the same data value as attribute $a$ at the current position, likewise for $d$ and $b$' can be expressed by $\multiC{a}{b} F^= ((\att{c}, \att{d}) \wedge p)$. 

However, already a restricted version of this extension is undecidable. We consider the operators $\X_{\att{\mathrm{a}},\att{\mathrm{b}}}$ and $\Y_{\att{\mathrm{a}},\att{\mathrm{b}}}$. Let the semantics of 
  $\X_{\att{\mathrm{a}},\att{\mathrm{b}}}$ be defined by 
$w,i\models \X_{\att{\mathrm{a}},\att{\mathrm{b}}}\varphi$ if there is a
$j>i$ with $\mdata{w}{a}{i}=\mdata{w}{a}{j}$ and
$\mdata{w}{b}{i}=\mdata{w}{b}{j}$ and for the smallest such $j$ it
holds $w,j\models\varphi$. The operator $\Y_{\att{a},\att{b}}$ is defined analogously.

\begin{theorem}\label{theo:multi-undec}
    \dataltl extended by the operators $\X_{\att{a},\att{b}}$ and $\Y_{\att{a},\att{b}}$ is undecidable on finite (or infinite) attributed words.
\end{theorem}

  \begin{proof}
    The proof is along the lines of Proposition 27 in \cite{BojanczykMSSD2006}. For the convenience of the reader, we sketch the proof.

    We reduce from the Post Correspondence Problem (PCP) which is defined by
    
      \problemdescr{PCP}{$(u_1, v_1), \ldots, (u_k, v_k) \in \Sigma^* \times \Sigma^*$}{Is there a non-empty sequence $(u_{i_1}, v_{i_1}), \ldots, (u_{i_n}, v_{i_n})$ such that $u_{i_1} \ldots u_{i_n} = v_{i_1} \ldots v_{i_n}$?} 

    Given a PCP $P$ we construct a \dataltl formula $\varphi_P$ using the operators $\X_{\att{a},\att{b}}$ and $\Y_{\att{a},\att{b}}$  such that there is a valid sequence for $P$ if and only if $\varphi_P$ is satisfiable. We can assume w.l.o.g. that if there is a valid sequence for $P$, then there is one of odd length.

    Let $P := (u_1, v_1), \ldots, (u_k, v_k) \in \Sigma^* \times \Sigma^*$. Then $\varphi_P$ uses the propositions $\Sigma \times \bar \Sigma$ where $\bar \Sigma := \{\bar \sigma \mid \sigma \in \Sigma\}$. 

    A valid sequence $(u_{i_1}, v_{i_1})\ldots (u_{i_n}, v_{i_n})$ of odd length for $P$ is mapped to an attributed word $w$ such that:
    \begin{itemize}
      \item[(1)] Every position of $w$ bears exactly one proposition and the word projection of $w$ is of the form 
      $u_{i_1} \bar v_{i_1} \ldots u_{i_n} \bar v_{i_n}$.
      \item[(2)] The attributes $a$ and $b$ are present at all positions and the data values of the attributes $a$ and $b$ for the word $u := u_{i_1} \ldots u_{i_n}$ are of the form \\
      $(d^a_1, d^b_1)(d^a_1, d^b_2)(d^a_2, d^b_2), \ldots, (d^a_{n-1}, d^b_{n}), (d^a_{n}, d^b_{n})$. The same for the word $\bar v:= \bar v_{i_1} \ldots \bar v_{i_n}$.
      \item[(3)] In $u := u_{i_1} \ldots u_{i_n}$ all values of attribute $a$ occur exactly twice, except for the value of 
      $a$ at the last position of $u$. Similarly all values of attribute $b$ occur exactly twice, except for the value of $b$ at the first position of $u$. The same holds for $\bar v:= \bar v_{i_1} \ldots \bar v_{i_n}$. 
      \item[(4)] Every pair $(d_a, d_b)$ of data values for the attributes $a$ and $b$ occurs exactly twice, once in $u$ and once in $\bar v$ and the position in $u$ is labeled by $\sigma$ if and only if the corresponding position in $\bar v$ is labeled by $\bar \sigma$.
    \end{itemize}
Note that conditions (2)-(4) ensure that $u = v'$, where $v'$ results from $\bar v$ by replacing every $\bar \sigma$ in $\bar v$ by $\sigma$.

    The first three properties can be checked easily by a \dataltl formula. Condition (4) can be checked using the additional operators: 
    
    $G\bigg(\bigvee_{\sigma \in \Sigma} \Big(\sigma \rightarrow \big((\X_{\att{\mathrm{a}},\att{\mathrm{b}}}\bar \sigma \wedge \neg \X_{\att{\mathrm{a}},\att{\mathrm{b}}}\X_{\att{\mathrm{a}},\att{\mathrm{b}}} \top \wedge \neg \Y_{\att{\mathrm{a}},\att{\mathrm{b}}} \top) \vee $ \\
     \mbox{ }\hfill $(\Y_{\att{\mathrm{a}},\att{\mathrm{b}}}\bar \sigma \wedge \neg \Y_{\att{\mathrm{a}},\att{\mathrm{b}}}\Y_{\att{\mathrm{a}},\att{\mathrm{b}}} \top \wedge \neg \X_{\att{\mathrm{a}},\att{\mathrm{b}}} \top)\big)\Big)\bigg) $
    $$\wedge$$
    $G\bigg(\bigvee_{\bar \sigma \in \bar\Sigma} \Big(\bar \sigma \rightarrow \big((\X_{\att{\mathrm{a}},\att{\mathrm{b}}} \sigma \wedge \neg \X_{\att{\mathrm{a}},\att{\mathrm{b}}}\X_{\att{\mathrm{a}},\att{\mathrm{b}}} \top \wedge \neg \Y_{\att{\mathrm{a}},\att{\mathrm{b}}} \top) \vee $ \\
  \mbox{ }\hfill  $ (\Y_{\att{\mathrm{a}},\att{\mathrm{b}}} \sigma \wedge \neg \Y_{\att{\mathrm{a}},\att{\mathrm{b}}}\Y_{\att{\mathrm{a}},\att{\mathrm{b}}} \top \wedge \neg \X_{\att{\mathrm{a}},\att{\mathrm{b}}} \top)\big)\Big)\bigg)$
    %$$\G  (\bigvee \Sigma \rightarrow (\F_{\att{a},\att{b}}\bigvee \bar \Sigma \leftrightarrow \neg \Y_{\att{a},\att{b}}\bigvee \bar \Sigma))
      %\wedge \G  (\bigvee \bar \Sigma \rightarrow (\F_{\att{a},\att{b}}\bigvee \Sigma \leftrightarrow \neg \Y_{\att{a},\att{b}} \bigvee \Sigma))$$\\
    \qed
  \end{proof}

\paragraph*{\dataltl with From-Now-On Operator} \label{sec:tuplecomp}

The \textit{from-now-on}-operator $\Now$ introduced in \cite{LaroussinieS95} restricts the range of past operators. For an attributed word $w =w_1 \ldots w_n$ and a position $i$ of $w$ let $\suf{w}{i} := w_i \ldots w_n$ be the suffix of $w$ starting at position $i$. The semantics of $\Now$ is then defined by
\begin{itemize}
\item $w,i \models \Now \varphi$ if $\suf{w}{i},1 \models \varphi$
\end{itemize}

\begin{theorem} \label{theo:undN}
\dataltl extended by the operator $\Now$ is undecidable on finite (or infinite) \attwords.
\end{theorem}  

\begin{proof}
    For technical reasons, we prove that \dataltl with the operator $\bar \Now$, the dual on $\Now$ is undecidable. For an attributed word $w =w_1 \ldots w_n$ and a position $i$ of $w$ let $\pre{w}{i} := w_1 \ldots w_i$ be the prefix of $w$ ending at position $i$. The semantics of $\bar \Now$ is then defined by
    \begin{itemize}
      \item $w,i \models \bar \Now \varphi$ if $\pre{w}{i},i \models \varphi$
    \end{itemize}


  As \dataltl is symmetric with respect to the availability of future and past operators, undecidability of \dataltl with $\Now$ follows from the undecidability of \dataltl with $\bar \Now$.


  The proof is by a reduction from the nonemptiness problem for
  Minsky two counter automata \cite{Minsky1967}.

A \textit{Minsky 2-CA} is a finite automaton equipped with two
counters $C_1$ and $C_2$. With each transition of the automaton a
\emph{counter action} is associated. In a counter action  a counter
can be incremented or decremented by 1 ($\inc_1$, $\inc_2$,
$\dec_1$, $\dec_2$) or counter can be tested for 0 ($\ifzero_1$,
$\ifzero_2$). Initially, both counters have the value 0. The semantics
is straightforward. If  a counter $i$ has value 0 a transition with a
$\dec_i$-action can not be applied. A transition with a $\ifzero_i$ action
can only be applied if counter $i$ is 0. 

It is well known that the emptiness problem for Minsky 2-CA is undecidable \cite{Minsky1967}.

Our reduction constructs, for every Minsky 2-CA $\calC$ an extended
\dataltl formula
$\varphi$ such that $L(\calC)\not=\emptyset$ if and only if $\varphi$
is satisfiable by a 1-\attword. We can assume without loss of generality that $\calC$ only
accepts if both counters are zero.

We encode runs of $\calC$ by
1-\attwords as follows. Each position $i$ carries two propositions, one is
the state of $\calC$ after step $i$   and the other the action in step
$i$. As in an accepting run there are, for each $i$ exactly as many
$\inc_i$ actions as there are $\dec_i$ actions we can assign data
values in a way such that each data value
\begin{itemize}
\item either occurs exactly once at an \ifzero-test or
\item once at an $\inc_i$ action and once at the corresponding\footnote{That is, if the first increments counter 1 from $m$ to
  $m+1$ the other is the action that decreases it back from $m+1$ to $m$.}
  $\dec_i$-action. 
\end{itemize}

It is not hard to write an \dataltl formula with the $\bar\Now$ operator that expresses that
\begin{enumerate}[(1)]
\item successive positions are consistent with respect to the
  transitions of $\calC$, the first position carries starting state and the
  final position carries an accepting state,
\item every data value only occurs once at an  \ifzero-test or
twice: once at a $\dec_i$ action and once at a smaller position with a
$\inc_i$-action, and
\item an $\ifzero_i$-action never occurs between an $\inc_i$-action
  and the $\dec_i$-action with the same data value.
\end{enumerate}

Note that condition (3) makes sure that an $\ifzero_i$-action only
occurs if counter $C_i$ is 0. Conditions (1) and (2) can be easily
expressed by \dataltl. 

Condition (3) can be expressed by the formula
\[
\bigwedge_{i=1}^2 \G  (\ifzero_i \ra \bar \Now\Hist(\inc_i \rightarrow \C{a} \CF \dec_i))
\]
\qed
\end{proof}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "start"
%%% ispell-local-dictionary: "english"
%%% End: 

